Grafting for Combinatorial Boolean Model using Frequent Itemset Mining

This paper introduces the combinatorial Boolean model (CBM), which is defined as the class of linear combinations of conjunctions of Boolean attributes. This paper addresses the issue of learning CBM from labeled data. CBM is of high knowledge interpretability but na\"{i}ve learning of it requires exponentially large computation time with respect to data dimension and sample size. To overcome this computational difficulty, we propose an algorithm GRAB (GRAfting for Boolean datasets), which efficiently learns CBM within the $L_1$-regularized loss minimization framework. The key idea of GRAB is to reduce the loss minimization problem to the weighted frequent itemset mining, in which frequent patterns are efficiently computable. We employ benchmark datasets to empirically demonstrate that GRAB is effective in terms of computational efficiency, prediction accuracy and knowledge discovery.

==> Definitions.tex <==
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\let\proof\relax
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
% \newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
% \newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

% \ifx\proof\undefined
% \newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
% \fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}[theorem]{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}

%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

\newcommand{\Omegabar}{\bar{\Omega}}

%%%% Symbols specific to this project %%%%%

\newcommand{\Poisson}{\mathrm{Poisson}}
\newcommand{\trank}{\text{rank}}
\newcommand{\otrank}{\overline{\text{rank}}}


==> experiments_0216.tex <==
\section{Experiments}
\label{sec:experiments}

We implemented our algorithm and conducted a set of experiments.
Our experiments are designed to clarify following benefits of our methods:
\begin{itemize}
\item Computational Efficiency
\item Model Complexity
\item Knowledge Discoverability
\end{itemize}

In order to select new features to be added, we used Linear time Closed itemset Miner (LCM) by ~\cite{Uno03,Uno04,Uno05}, which is one of backtracking-based frequent itemset mining algorithms.
Of course, we may apply any other WFIM algorithms to this purpose.

計算の実行環境。
OS: CentOS 6.4
RAM: 96GB
CPU: Intel(R) Xeon(R) CPU           X5690  @ 3.47GHz

\subsection{Evaluation of computation time}
In order to evaluate efficiency of GRAB from the perspective of computation efficiency, we measured computation time required to train CBM models by GRAB 
and other algorithms on a benchmark dataset.
We focused on two aspects: benefits of using grafting algorithm and benefits of using WFIM algorithm.
Therefore, as comparison methods, the following two are used:
\begin{enumerate}
\item{Expansion + $L_1$-regularized logistic regression\\}
first convert dataset using all the possible features~$\phi\in\Phi^{(k)}$ (expansion),
and then we solve this combinatorial linear problem as $L_1$-regularized logistic regression problem on the converted dataset.
\item{Grafting + na\"{\i}ve feature selection\\}
uses grating algorithm, but not WFIM.
In order to calculate \eqref{eq:grafting_weight_choice},
we exhaustively search all the possible features~$\phi\in\Phi^{(k)}$.
\end{enumerate}
In this experiment, the logistic loss function $\ell(f(\bm{x}), y)\triangleq -\log\rbr{1/\rbr{1+\exp\rbr{-yf(\bm{x}}}}$ 
is used as a loss function of combinatorial boolean model.
\textcolor{red}{
As a benchmark, we use a1a dataset~\cite{a1a},
which has 32,561 records and 123 features.
We trained combinatorial boolean model with $C=0.1, 1$ and $k=1,2,3,4,5,6,\infty$ using each algorithm,
and measure calculation time.
The results are shown on the table~\ref{tab:time}.
}
\begin{table*}[htbp]
\caption{
Comparison of computation time (sec) on a1a dataset:
the bracketed values at \textit{Expand+$L_1$-regularized Logistic Regression}
mean the elapsed times to solve $L_1$-regularized logistic regression.
}
\label{tab:time}
\begin{center}
\begin{tabular}{|r||r|r|r|r|r|r|} \hline
           & \multicolumn{2}{|c|}{GRAB} & \multicolumn{2}{|c|}{Grafting + na\"{i}ve feature selection} & \multicolumn{2}{|c|}{Expansion + $L_1$-regularized Logistic Regression} \\ \hline
           & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$}  & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} \\ \hline
$k=1$      & 2.1 & 1.7 & \ \ \ \ \ \ \ \ \ \ 5.3 & 4.0 & 3.0E-1\ (1.4E-1) & 2.4E-2\ (8.5E-2) \\ \hline
$k=2$      & 4.5 & 5.8E+1 & 3.2E+2 & 2.9E+2 & 3.8\ (3.0E-1) & 3.8\ (3.2E-1) \\ \hline
$k=3$      & 8.7 & 2.1E+1 & 1.3E+4 & 1.2E+4 & 5.5E+1\ (9.8E-1) & 5.5E+1\ (1.1) \\ \hline
$k=4$      & 1.3E+1 & 4.1E+1 & >1 day        & >1 day        & 4.7E+2\ (1.4) & 4.7E+2\ (1.9) \\ \hline
$k=5$      & 1.5E+1 & 9.2E+1 & >1 day        & >1 day        & 2.3E+3\ (5.1) & 2.3E+3\ (5.2) \\ \hline
$k=6$      & 1.7E+1 & 1.4E+2 & >1 day        & >1 day        & 7.6E+3\ (1.3E+1) & 7.6E+3\ (1.1E+1) \\ \hline
$k=\infty$ & 2.3E+1 & 2.9E+2 & >1 day        & >1 day        & 5.6E+4\ (9.2E+1) & 5.6E+4\ (9.1E+1) \\ \hline
\end{tabular}
\end{center}
\end{table*}

\textcolor{red}{
First, it is obvious that the computation time of GRAB is much less than that of Grafting+Na\"{\i}ve feature selection.
This result shows that WFIM can efficiently select the feature~$\phi\in\Phi^{(k)}$.
Next, let us compare the results of GRAB and Expansion+$L_1$-regularized logistic regression.
Although $L_1$-regularized logistic regression optimizes parameters more rapidly than GRAB,
expansion step takes much longer time than the whole of GRAB algorithm.
Therefore, GRAB is more efficient to learn combinatorial boolean model
than expansion+$L_1$-regularized logistic regression.
}

\subsection{Evaluation of prediction accuracy}
\textcolor{red}{
In order to evaluate GRAB's prediction performance,
we conduct experiments on the following benchmark datasets:
\begin{enumerate}
\item
\textbf{a1a}~\cite{a1a}: has 32,561 records and 123 features for each data.
This dataset is obtained by preprocessing  Adult dataset~\cite{Adult},
which has 6 continuous and 8 categorical features.
We devide the total data into 30,000 training data and 2,561 test data.
\item
\textbf{cod-rna}~\cite{cod-rna}: is a dataset for the problem of detecting non-coding RNAs from features of base sequences.
Since all of 8 features consist of continuous values,
we binarize each feature by the following procedure:
we devide the interval from the minimum value to the maximum value into 30 equal parts,
and indicate which section the value enters by a flag.
Thus, a binary dataset with 240 features is obtained, each data of which has just 8 non-zero features.
We use 300,000 data for training and 31,152 for test.
\item
\textbf{covtype.binary}~\cite{covtype.binary}: is a dataset obtained by transforming Covertype dataset~\cite{}
from multiclass into binary class.
The original covertype dataset has 581,012 instances with 54 cartographic attributes,
10 of which are quantitative ones and the rest are binary,
and forest cover type categorized by seven as labels.
For CBM, we binarize all the quantitative attributes in the same way as cod-rna dataset.
We use 500,000 data for training and 81,012 for test.
\if 0
\item
\textbf{traffic}: was collected from 1,727 intersections in Tokyo,
873 of which are dangerous road points where more than 4 traffic accidents occurred at 2012 (positive example),
and the rest are other non-risky road points (negative example).
At each target intersection, we collect binary of categorical features such as signal type and presence of sidewalks from all the connected road.
For example, when road feature vector
Our task is to predict whether road points are risky or not
from information of intersection structures, such as signal types, presence of sidewalks and so on.
\fi
\end{enumerate}
As comparison learning models, we adopt support vector classification (SVC)
with two kinds of kernel functions, polynomial kernel (\textit{poly}) and radial basis function kernel (\textit{rbf}),
both of which are widely used to classification tasks.
We formulate polynomial kernel as $k(\bm{x},\bm{x}')=\rbr{\gamma \bm{x}^\top\bm{x}'+\rbr{1-\gamma}}^d$,
where $d\in\mathbb{N}_+$ and $\gamma\in (0,1]$ are hyperparameters,
and radial basis function kernel as $k(\bm{x},\bm{x}')=\exp\rbr{\frac{1}{2\gamma}\|\bm{x}-\bm{x}'\|^2_2}$,
where $\gamma>0$ is a hyperparameter.
}

\textcolor{red}{
We adopt logistic loss and $L_2$-hinge loss as loss functions of CBM.
$L_2$-hinge loss function is defined as follows:
\begin{align*}
\ell(f(\bm{x}), y)\triangleq \begin{cases}
\rbr{1-yf(\bm{x})}^2 & (1-yf(\bm{x})<0) \\
0 & (\text{otherwise.})
\end{cases}
.
\end{align*}
It should be noted that WFIM procedure of GRAB can be accelerated
when we use $L_2$-hinge loss,
since it holds that $\partial \ell(\bm{x}_i,y_i)/\partial f^{(k)}(\bm{x})$,
which is the $i$-th transaction weight of WFIM,
is $0$ for all $i$ that satisfy $1-y_if(\bm{x}_i)\geq 0$
and we can remove them from the transaction database.
On each benchmark dataset,
We compare test accuracy of
1: Polynomial kernel SVC with $d=1$ and $3$,
2: RBF kernel SVC,
3: Logistic loss CBM with $k=1,3$ and $\infty$, and
4: $L_2$-hinge loss CBM with $k=1,3$ and $\infty$.
After training each model with $C=10^{-3},10^{-2},\ldots,10^3$
and $\gamma=0.1,0.2,\ldots,1$ for SVC on training data,
we choose the model with the highest accuracy on test data
as the final output.
}

\textcolor{red}{
The accuracy score of each model on each benchmark dataset
is summarized on Table~\ref{tab:accuracy}.
First, let us explain the result on a1a dataset.
It can be seen that each method including the cases of Poly with $d=1$
and GRAB with $k=1$ achieves about the same accuracy.
From this observation, we can say that
linear models can sufficiently predict a1a dataset.
In terms of computation time, logistic loss GRAB with $k=3$ achieves
more than 10 times faster learning than polynomial kernel SVC with $d=3$.
}

\textcolor{red}{
Next, the results on cod-rna dataset are shown at Table~\ref{tab:accuracy}\subref{tab:accuracy_cod-rna}.
We can observe that the accuracies of SVC on the binarized dataset are much greater than those on the raw one.
This can be considered to be due to the fact that
cod-rna dataset approaches linearly separable data by binarization.
Comparing the results of $L_2$-hinge loss GRAB with $k=1$ and $\infty$,
the case of $k=\infty$ improves the accuracy more than $1\%$.
From this result, it can be also said that combinatorial features are significance on prediction of cod-rna dataset.
In terms of accuracy, poly with $d=3$ on the binarized data, which is the best in SVCs,
is almost the same as $L_2$-hinge loss GRAB with $k=\infty$, which is the best in GRABs.
However, the computation time of the best in GRABs is less than one hundredth of that of the best in SVCs.
This is because binarized cod-rna dataset posses very high sparsity such that the number of nonzero elements per record is just eight out of 240,
and WFIM can be executed very rapidly.
}

\textcolor{red}{
Finally, we show the results on covtype.binary dataset at Table~\ref{tab:accuracy}\subref{tab:accuracy_covtype.binary}.
As in the case of cod-rna dataset, we can see that binarization improves the accuracies of SVCs.
It can be also seen that combinatorial features greatly contribute to prediction of covtype.binary dataset.
}
\if 0
次に、cod-rnaデータセットでの結果に移る。
まずSVCによるRawデータとBinarizedデータの結果を比較すると、二値化したものの方が高い精度を示していることがわかる。
これは二値化したことにより、データの線型性が向上したためだと考えられる。
またGRABに関しては$k=1$と$\infty$の結果を比較すると、精度が1\%ほど向上していることがわかる。
このことから、特徴量の組合せがcod-rnaの予測に有効であることがわかる。
SVCに関してはpolyかつ$d=3$で、GRABに関しては$L_2$-logistic lossかつ$k=\infty$でそれぞれ
精度が最良となり、量手法ともほぼ同様の値となっていることがわかる。
しかしながら計算時間の点ではGRABの方が100倍以上高速に計算できていることが確認できる。
これは、二値化することによって次元数が8から240に増加しているが、データ1件中の非ゼロ要素数は
8しかなく、データのsparse性が非常に高く、高速にWFIMが実行できるからだと考えられる。

最後にcovtype.binaryでの結果を見ていく。
まずcod-rnaと同様に二値化することにより精度が向上する傾向が見られる。
また、Polyの$d=1$と$3$の場合及び、GRABの$k=1$とそれ以外の結果から分かる通り、
特徴量の組み合わせを考慮することで大きく予測精度を向上できている。
予測精度に関しては…
また計算時間に関しては…
cod-rnaの計算時間がSVC
\fi

\begin{table*}[htbp]
\caption{
Comparison of accuracy (\%) on benchmark datasets:
the terms \textit{Raw} and \textit{Binarized} mean that
we used the original and the binarized dataset, respectively,
as a training data.
The row \textit{Time} shows the elapsed time (sec) of each method
when the number of training data is the maximum.
}
\label{tab:accuracy}
\begin{center}
\subfloat[a1a \label{tab:accuracy_a1a}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|} \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
7,500 & 85.2 & 85.3 & 85.2 & 84.9 & 84.7 & 84.9 & 84.9 & 85.3 & 84.5 \\ \hline
30,000 & 85.4 & 85.3 & 85.2 & 85.0 & 85.5 & 85.5 & 85.1 & 85.5 & 84.3 \\ \hline\hline
Time (sec) & 2.3E+2 & 1.0E+2 & 1.4E+2 & 1.4 & 6.9 & 1.7E+1 & 1.2 & 1.4E+1 & 5.0 \\ \hline
\end{tabular}
}

\subfloat[cod-rna \label{tab:accuracy_cod-rna}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 88.9 & 88.8 & 89.3 & 95.6 & 96.0 & 96.0 & 95.5 & 95.9 & 95.9 & 95.5 & 96.0 & 96.0 \\ \hline
100,000 & 89.0 & 88.9 & 90.1 & 95.7 & 96.3 & 96.3 & 95.6 & 96.0 & 96.0 & 95.6 & 96.3 & 96.3 \\ \hline
300,000 & & 89.0 & 93.0 & 95.7 & 96.6 & 96.4 & 95.6 & 96.5 & 96.5 & 95.6 & 96.6 & 96.7 \\ \hline\hline
Time (sec) & & 3.8E+3 & & 8.0E+3 & 1.4E+4 & 1.1E+4 & 6.4E+1 & 2.1E+2 & 1.1E+2 & 1.5E+1 & 8.8E+1 & 1.1E+2 \\ \hline
\end{tabular}
}

\subfloat[covtype.binary \label{tab:accuracy_covtype.binary}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 76.0 & 82.0 & 86.1 & 74.4 & 86.8 & 87.6 & 76.9 & 86.7 & 86.9 & 76.9 & 86.5 & 86.6 \\ \hline
100,000 & 76.1 & 82.4 & 87.0 & & 90.6 & 91.2 & 77.0 & 90.8 & 90.9 & 77.0 & 90.4 & 90.6 \\ \hline
500,000 & & & & > 1 day & > 1 day & > 1 day & 76.9 & 94.1 & 94.3 & 77.0 & 94.3 & 94.7 \\ \hline\hline
Time (sec) & & & & & & & 6.6E+1 & 3.7E+3 & 4.7E+3 & 3.8E+1 & 2.6E+3 & 3.6E+3 \\ \hline
\end{tabular}
}
\end{center}
\end{table*}

\subsection{Evaluation of interpretability}
\textcolor{red}{
We evaluate interpretability of GRAB by acquiring knowledge from the predictor.
Weights with large absolute values can be interpreted as knowledge,
since they greatly affect the prediction results.
First, we show weights with large absolute values,
which are obtained by training GRAB with $L_2$-hinge loss and $k=3$ on a1a dataset,
on Table~\ref{tab:a1a_knowledge}.
\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from a1a dataset.
}
\label{tab:a1a_knowledge}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
-0.581 & (Unmarried) \\ \hline
0.544 & (Unmarried) \& (No monetary capital losses) \\ \hline
0.455 & (Self-employment not inc.) \& (Asian-Pacific Islander) \& (Large monetary capital gains) \\ \hline
-0.432 & (No capital gains) \& (No capital losses) \\ \hline
0.390 & (Large final weight) \& (Other race) \& (From India) \\ \hline
0.353 & (Divorced) \\ \hline
0.325 & (Craft-repair) \& (No monetary capital gains) \& (Long average hours per week worked) \\ \hline
0.320 & (Never married) \& (No monetary capital losses) \& (From Puerto-Rico) \\ \hline
-0.291 & (Divorced) \& (Exec-managerial) \& (Short average hours per week worked) \\ \hline
0.272 & (Married with civilian spouse) \& (Machine operator inspector) \& (Large monetary capital gains) \\ \hline
\end{tabular}
\end{table*}
}

\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from covtype.binary dataset.
}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
1.997469 & Elevation(10) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
1.932653 & Elevation(11) \& Horizontal Distance to nearest wildfire ignition point(30) \\ \hline
1.904661 & Elevation(18) \& Horizontal Distance to nearest roadway(17) \& Horizontal Distance to nearest wildfire ignition points(9) \\ \hline
1.887015 & Horizontal Distance to nearest roadway(12) \& Horizontal Distance to nearest wildfire ignition pints(11) \& Leighcan family, till substratum - Typic Cryaquolls complex. \\ \hline
1.810542 & Horizontal Distance to nearest roadway(9) \& Horizontal Distance to nearest wildfire ignition point(278) \& Rawah Wilderness Area(301) \\ \hline
1.775597 & Horizontal Distance to nearest wildfire ignition points(12) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.715680 & Horizontal Distance to nearest wildfire ignition points(11) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.636024 & Elevation(9) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
-1.627047 & Comanche Peak Wilderness Area \\ \hline
1.609355 & Elevation(20) \& Horizontal Distance(7) \& Horizontal Distance to nearest wildfire ignition points(6) \\ \hline
1.601753 & Elevation(11) \\ \hline
1.600297 & Elevation(7) \& Horizontal Distance to nearest roadway(2) \& Horizontal Distance to nearest wildfire ignition points(275) \\ \hline
1.571094 & Elevation(13) \\ \hline
1.565210 & Horizontal Distance to nearest roadway(13) \& Horizontal Distance to nearest wildfire ignition points(13) \& Neota Wilderness Area \\ \hline
\end{tabular}
\end{table*}

polymonial kernel is difficult to hyper-tune

==> experiments_0217.tex <==
\section{Experiments}
\label{sec:experiments}

We implemented our algorithm GRAB to 
evaluate the computational complexity, prediction accuracy, and knowledge interpretability.
In order to select new features to be added, we used Linear time Closed itemset Miner (LCM) by ~\cite{Uno03,Uno04,Uno05}, which is one of backtracking-based FIM  algorithms.
%Of course, we may apply any other WFIM algorithms to this purpose.

計算の実行環境。
OS: CentOS 6.4
RAM: 96GB
CPU: Intel(R) Xeon(R) CPU           X5690  @ 3.47GHz

\subsection{Evaluation of Computation Time}
In order to evaluate the computational efficiency of GRAB, 
we employed benchmark data sets to compare GRAB with other methods in terms of  computation time required for learning CBM.
We investigated how effective the grafting algorithm and WFIM were respectively.
To this end, as methods for comparison, we employed the following two combinations:
\begin{enumerate}
\item{Expansion + $L_1$-regularized logistic regression\\}
In this combination, we first expand a data set so that  all possible features are employed to express it ~$\phi\in\Phi^{(k)}$ (expansion).
We then learn combinatorial linear models on the expanded data set within the $L_1$-regularized logistic regression framework.
\item{Grafting + na\"{\i}ve feature selection\\}
We employ the grating algorithm, without combing it with WFIM.
In it we calculate \eqref{eq:grafting_weight_choice} by searching exhaustively over  the set of all features~$\phi\in\Phi^{(k)}$.
\end{enumerate}

In this experiment, we used the logistic loss function $\ell(f(\bm{x}), y)\triangleq -\log\rbr{1/\rbr{1+\exp\rbr{-yf(\bm{x}}}}$ 
as a loss function for learning CBM.
As a benchmark data set, we used a1a dataset~\cite{a1a},
which has 32,561 records and 123 features.
We conduced learning CBM with $C=0.1, 1$ and $k=1,2,3,4,5,6,\infty$ 
for the respective algorithms.
The results on computation time are shown in Table~\ref{tab:time}.

\begin{table*}[htbp]
\caption{
Comparison of computation time (sec) on a1a dataset:
the bracketed values at \textit{Expand+$L_1$-regularized Logistic Regression}
mean the elapsed times to solve $L_1$-regularized logistic regression.
}
\label{tab:time}
\begin{center}
\begin{tabular}{|r||r|r|r|r|r|r|} \hline
           & \multicolumn{2}{|c|}{GRAB} & \multicolumn{2}{|c|}{Grafting + na\"{i}ve feature selection} & \multicolumn{2}{|c|}{Expansion + $L_1$-regularized Logistic Regression} \\ \hline
           & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$}  & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} \\ \hline
$k=1$      & 2.1 & 1.7 & \ \ \ \ \ \ \ \ \ \ 5.3 & 4.0 & 3.0E-1\ (1.4E-1) & 2.4E-2\ (8.5E-2) \\ \hline
$k=2$      & 4.5 & 5.8E+1 & 3.2E+2 & 2.9E+2 & 3.8\ (3.0E-1) & 3.8\ (3.2E-1) \\ \hline
$k=3$      & 8.7 & 2.1E+1 & 1.3E+4 & 1.2E+4 & 5.5E+1\ (9.8E-1) & 5.5E+1\ (1.1) \\ \hline
$k=4$      & 1.3E+1 & 4.1E+1 & >1 day        & >1 day        & 4.7E+2\ (1.4) & 4.7E+2\ (1.9) \\ \hline
$k=5$      & 1.5E+1 & 9.2E+1 & >1 day        & >1 day        & 2.3E+3\ (5.1) & 2.3E+3\ (5.2) \\ \hline
$k=6$      & 1.7E+1 & 1.4E+2 & >1 day        & >1 day        & 7.6E+3\ (1.3E+1) & 7.6E+3\ (1.1E+1) \\ \hline
$k=\infty$ & 2.3E+1 & 2.9E+2 & >1 day        & >1 day        & 5.6E+4\ (9.2E+1) & 5.6E+4\ (9.1E+1) \\ \hline
\end{tabular}
\end{center}
\end{table*}


We first observe that the computation time for GRAB is significantly smaller than that of of Grafting+Na\"{\i}ve feature selection.
It implies that WFIM was so efficient that it could  select the feature~$\phi\in\Phi^{(k)}$.
We then compare GRAB with Expansion+$L_1$-regularized logistic regression to 
have the following observation:
$L_1$-regularized logistic regression solved the parameter optimization problem more quickly than GRAB. 
However, the expansion step took much longer time than the whole procedure of GRAB.
It implies that GRAB learned CBM significantly more effectively than  cexpansion+$L_1$-regularized logistic regression.


\subsection{Evaluation of prediction accuracy}

In order to evaluate GRAB's prediction performance,
we conducted experiments for the following benchmark datasets:
\begin{enumerate}
\item
\textbf{a1a}~\cite{a1a}: It has 32,561 records and 123 attributes for each data.
This dataset is obtained by preprocessing  Adult dataset~\cite{Adult},
which has 6 continuous and 8 categorical features.
We divided the total data into 30,000 training data and 2,561 test data.
\item
\textbf{cod-rna}~\cite{cod-rna}: It is a dataset for the problem of detecting non-coding RNAs from attributes of base sequences.
Since all of  the 8 attributes are real-valued,
we transformed  each attribute into a binary one as follows:
We divided the interval from the minimum value to the maximum value into 30 cells of equal length.
We expressed each attribute in a binary form by indicating which section its value fell into.
Thus, a binary dataset with 240 attributes was obtained.
Each data in it was specified by  8 non-zero attributes.
We used 300,000 data for training and 31,152 for test.
\item
\textbf{covtype.binary}~\cite{covtype.binary}:
It is a dataset obtained by transforming Covertype dataset~\cite{}
with multi labels into the one with binary labels.
The original Covertype dataset has 581,012 instances with 54 cartographic attributes,
10 of which are quantitative ones and the rest are binary,
and forest cover type categorized by seven as labels.
We binarized all the quantitative attributes in the same way as cod-rna dataset.
We used 500,000 data for training and 81,012 for test.
\if 0
\item
\textbf{traffic}: was collected from 1,727 intersections in Tokyo,
873 of which are dangerous road points where more than 4 traffic accidents occurred at 2012 (positive example),
and the rest are other non-risky road points (negative example).
At each target intersection, we collect binary of categorical features such as signal type and presence of sidewalks from all the connected road.
For example, when road feature vector
Our task is to predict whether road points are risky or not
from information of intersection structures, such as signal types, presence of sidewalks and so on.
\fi
\end{enumerate}
As methods for comparison, we employed support vector classification (SVC)
with two types of kernel functions: polynomial kernel (\textit{poly}) and radial basis function kernel (\textit{rbf}),
both of which have extensively been used for the purpose of classification.
The polynomial kernel is defined as $k(\bm{x},\bm{x}')=\rbr{\gamma \bm{x}^\top\bm{x}'+\rbr{1-\gamma}}^d$,
where $d\in\mathbb{N}_+$ and $\gamma\in (0,1]$ are hyper parameters,
and radial basis function kernel is defined as $k(\bm{x},\bm{x}')=\exp\rbr{\frac{1}{2\gamma}\|\bm{x}-\bm{x}'\|^2_2}$,
where $\gamma>0$ is a hyper parameter.


We employed the logistic loss  and the $L_2$-hinge loss as loss functions for learning CBM.
The $L_2$-hinge loss function is defined as:
\begin{align*}
\ell(f(\bm{x}), y)\triangleq \begin{cases}
\rbr{1-yf(\bm{x})}^2 & (1-yf(\bm{x})<0) ,\\
0 & (\text{otherwise.})
\end{cases}
\end{align*}
Note that the WFIM procedure in GRAB can be accelerated
by using the $L_2$-hinge loss.
This is because it holds $\partial \ell(\bm{x}_i,y_i)/\partial f^{(k)}(\bm{x})$,
which is the $i$-th transaction weight of WFIM,
is $0$ for all $i$ satisfying $1-y_if(\bm{x}_i)\geq 0$
and we can remove them from the transaction database.
For each of the benchmark datasets,
we compared  prediction accuracies of
\begin{enumerate}
\item Polynomial kernel SVC with $d=1$ and $3$,
\item RBF kernel SVC,
\item Logistic loss CBM with $k=1,3$ and $\infty$, 
\item $L_2$-hinge loss CBM with $k=1,3$ and $\infty$.
\end{enumerate}
For each of the algorithms,  
after learning models with $C=10^{-3},10^{-2},\ldots,10^3$ for CBM
and with $\gamma=0.1,0.2,\ldots,1$ for SVC from training data,
we selected the model with the highest accuracy on test data.
%as the final output.


Table~\ref{tab:accuracy} shows the accuracies of the respective algorithms.
From the results on a1a dataset, we see that GRAB with $k=1$ is 
almost comparable to Poly with $d=1$,
\textcolor{red}{
while the former finished training more than 100 times faster than the latter.
}
%while the time complexity of the former is ***  smaller than the latter.
%などの文がほしい
This implies that linear models are accurate enough for the prediction with a1a dataset.
The time complexity of logistic loss GRAB with $k=3$ 
was more than 10 times higher than polynomial kernel SVC with $d=3$.

From the results on cod-rna dataset shown in Table~\ref{tab:accuracy}\subref{tab:accuracy_cod-rna}, 
we observe that the accuracies of SVC on the binarized dataset are much greater than those on the raw one.
The reason for this may be that
cod-rna dataset got almost linearly separable by means of binarization.
$L_2$-hinge loss GRAB with  $k=\infty$ is more than $1\%$ more accurate than that with $k=1$. 
This implies that combinatorial features are effective for the prediction with cod-rna dataset.
Poly with $d=3$ on the binarized data, which achieved the highest accuracy among the SVC family, was almost comparable to $L_2$-hinge loss GRAB with $k=\infty$, 
which achieved the  highest accuracy among GRAB family.
However, the computation time of the best in GRABs was less than one hundredth of that of the best in SVCs.
This is because binarized cod-rna dataset was of high sparsity in the sense that the number of nonzero elements per record was just eight out of 240,
and WFIM was  executed very rapidly.
}


From the results on covtype.binary dataset shown in  Table~\ref{tab:accuracy}\subref{tab:accuracy_covtype.binary}, 
we see that  binarization contributed to the improvement of  accuracies of SVCs.
This was similar to the case of cod-rna.
We also see that combinatorial features greatly contributed to the prediction with covtype.binary dataset.
%計算量の比較も結果がでたら上の要領で書くべし

\if 0
次に、cod-rnaデータセットでの結果に移る。
まずSVCによるRawデータとBinarizedデータの結果を比較すると、二値化したものの方が高い精度を示していることがわかる。
これは二値化したことにより、データの線型性が向上したためだと考えられる。
またGRABに関しては$k=1$と$\infty$の結果を比較すると、精度が1\%ほど向上していることがわかる。
このことから、特徴量の組合せがcod-rnaの予測に有効であることがわかる。
SVCに関してはpolyかつ$d=3$で、GRABに関しては$L_2$-logistic lossかつ$k=\infty$でそれぞれ
精度が最良となり、量手法ともほぼ同様の値となっていることがわかる。
しかしながら計算時間の点ではGRABの方が100倍以上高速に計算できていることが確認できる。
これは、二値化することによって次元数が8から240に増加しているが、データ1件中の非ゼロ要素数は
8しかなく、データのsparse性が非常に高く、高速にWFIMが実行できるからだと考えられる。

最後にcovtype.binaryでの結果を見ていく。
まずcod-rnaと同様に二値化することにより精度が向上する傾向が見られる。
また、Polyの$d=1$と$3$の場合及び、GRABの$k=1$とそれ以外の結果から分かる通り、
特徴量の組み合わせを考慮することで大きく予測精度を向上できている。
予測精度に関しては…
また計算時間に関しては…
cod-rnaの計算時間がSVC
\fi

\begin{table*}[htbp]
\caption{
Comparison of accuracy (\%) on benchmark datasets:
the terms \textit{Raw} and \textit{Binarized} mean that
we used the original and the binarized dataset, respectively,
as a training data.
The row \textit{Time} shows the elapsed time (sec) of each method
when the number of training data is the maximum.
}
\label{tab:accuracy}
\begin{center}
\subfloat[a1a \label{tab:accuracy_a1a}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|} \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
7,500 & 85.2 & 85.3 & 85.2 & 84.9 & 84.7 & 84.9 & 84.9 & 85.3 & 84.5 \\ \hline
30,000 & 85.4 & 85.3 & 85.2 & 85.0 & 85.5 & 85.5 & 85.1 & 85.5 & 84.3 \\ \hline\hline
Time (sec) & 2.3E+2 & 1.0E+2 & 1.4E+2 & 1.4 & 6.9 & 1.7E+1 & 1.2 & 1.4E+1 & 5.0 \\ \hline
\end{tabular}
}

\subfloat[cod-rna \label{tab:accuracy_cod-rna}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 88.9 & 88.8 & 89.3 & 95.6 & 96.0 & 96.0 & 95.5 & 95.9 & 95.9 & 95.5 & 96.0 & 96.0 \\ \hline
100,000 & 89.0 & 88.9 & 90.1 & 95.7 & 96.3 & 96.3 & 95.6 & 96.0 & 96.0 & 95.6 & 96.3 & 96.3 \\ \hline
300,000 & 89.4 & 89.0 & 93.0 & 95.7 & 96.6 & 96.4 & 95.6 & 96.5 & 96.5 & 95.6 & 96.6 & 96.7 \\ \hline\hline
Time (sec) & 3.0E+3 & 3.8E+3 & 5.3E+3 & 8.0E+3 & 1.4E+4 & 1.1E+4 & 6.4E+1 & 2.1E+2 & 1.1E+2 & 1.5E+1 & 8.8E+1 & 1.1E+2 \\ \hline
\end{tabular}
}

\subfloat[covtype.binary \label{tab:accuracy_covtype.binary}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 76.0 & 82.0 & 86.1 & 74.4 & 86.8 & 87.6 & 76.9 & 86.7 & 86.9 & 76.9 & 86.5 & 86.6 \\ \hline
100,000 & 76.1 & 82.4 & 87.0 & 74.1 & 90.6 & 91.2 & 77.0 & 90.8 & 90.9 & 77.0 & 90.4 & 90.6 \\ \hline
500,000 & & & & - & - & - & 76.9 & 94.1 & 94.3 & 77.0 & 94.3 & 94.7 \\ \hline\hline
Time (sec) & & & & > 1 day & > 1 day & > 1 day & 6.6E+1 & 3.7E+3 & 4.7E+3 & 3.8E+1 & 2.6E+3 & 3.6E+3 \\ \hline
\end{tabular}
}
\end{center}
\end{table*}

\subsection{Evaluation of interpretability}
\textcolor{red}{
We evaluate interpretability of GRAB by acquiring knowledge from the predictor.
Weights with large absolute values can be interpreted as knowledge,
since they greatly affect the prediction results.
First, we show weights with large absolute values,
which are obtained by training GRAB with $L_2$-hinge loss and $k=3$ on a1a dataset,
on Table~\ref{tab:a1a_knowledge}.
\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from a1a dataset.
}
\label{tab:a1a_knowledge}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
-0.581 & (Not in family) \\ \hline
0.544 & (Not in family) \& (No monetary capital losses) \\ \hline
0.455 & (Self-employment (not inc.)) \& (Unmarried) \& (Have monetary capital gains) \\ \hline
-0.432 & (Female) \& (No monetary capital gains) \& (No monetary capital losses) \\ \hline
0.390 & (Low final weight) \& (Asian Pacific Islander) \& (From Japan) \\ \hline
0.353 & (High education number) \\ \hline
0.325 & (Married AF spouse) \& (No monetary capital gains) \& (From United States) \\ \hline
0.320 & (Married civ spouse) \& (No monetary capital losses) \& (From Canada) \\ \hline
-0.291 & (High education number) \& (Other service) \& (Middle average hours per week worked) \\ \hline
0.272 & (Slightly higher education number) \& (Prof specialty) \& (Have monetary capital gains) \\ \hline
\end{tabular}
\end{table*}
}

\if 0
\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from covtype.binary dataset.
}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
1.997469 & Elevation(10) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
1.932653 & Elevation(11) \& Horizontal Distance to nearest wildfire ignition point(30) \\ \hline
1.904661 & Elevation(18) \& Horizontal Distance to nearest roadway(17) \& Horizontal Distance to nearest wildfire ignition points(9) \\ \hline
1.887015 & Horizontal Distance to nearest roadway(12) \& Horizontal Distance to nearest wildfire ignition pints(11) \& Leighcan family, till substratum - Typic Cryaquolls complex. \\ \hline
1.810542 & Horizontal Distance to nearest roadway(9) \& Horizontal Distance to nearest wildfire ignition point(278) \& Rawah Wilderness Area(301) \\ \hline
1.775597 & Horizontal Distance to nearest wildfire ignition points(12) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.715680 & Horizontal Distance to nearest wildfire ignition points(11) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.636024 & Elevation(9) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
-1.627047 & Comanche Peak Wilderness Area \\ \hline
1.609355 & Elevation(20) \& Horizontal Distance(7) \& Horizontal Distance to nearest wildfire ignition points(6) \\ \hline
1.601753 & Elevation(11) \\ \hline
1.600297 & Elevation(7) \& Horizontal Distance to nearest roadway(2) \& Horizontal Distance to nearest wildfire ignition points(275) \\ \hline
1.571094 & Elevation(13) \\ \hline
1.565210 & Horizontal Distance to nearest roadway(13) \& Horizontal Distance to nearest wildfire ignition points(13) \& Neota Wilderness Area \\ \hline
\end{tabular}
\end{table*}
\fi

polymonial kernel is difficult to hyper-tune

==> experiments_0218.tex <==
\section{Experiments}
\label{sec:experiments}

We implemented our algorithm GRAB to 
evaluate its computational complexity, prediction accuracy, and knowledge interpretability.
In order to select new features to be added, we used Linear time Closed itemset Miner (LCM) by ~\cite{Uno03,Uno04,Uno05}, which is one of backtracking-based FIM  algorithms. All experiments below are executed by Linux (CentOS 6.4) machines 
with 94GB memory and Intel(R) Xeon(R) Processor X5690 @ 3.47GHz.

%計算の実行環境。
%OS: CentOS 6.4
%RAM: 96GB
%CPU: Intel(R) Xeon(R) CPU           X5690  @ 3.47GHz


\subsection{Evaluation of Computation Time}
In order to evaluate the computational efficiency of GRAB, 
we employed benchmark data sets to compare GRAB with other methods.
% in terms of  computation time required for learning CBM.
We investigated how effective the grafting algorithm and WFIM were respectively.
To this end, as methods for comparison, we employed the following two combinations:
\begin{enumerate}
\item{{\em Expansion + $L_1$-regularized logistic regression:}\\}
In this combination, we first expand a data set so that  all possible features are employed to express $\phi\in\Phi^{(k)}$ ({\em expansion}).
We then learn combinatorial linear models on the expanded data set within the $L_1$-regularized logistic regression framework.
\item{{\em Grafting + na\"{\i}ve feature selection:}\\}
I this combination we employ the grating algorithm, without combing it with WFIM. 
In it we calculate \eqref{eq:grafting_weight_choice} by searching exhaustively over  the set of all features~$\phi\in\Phi^{(k)}$.
\end{enumerate}

In our experiment, we used the logistic loss function $\ell(f(\bm{x}), y)\triangleq -\log\rbr{1/\rbr{1+\exp\rbr{-yf(\bm{x}}}}$ 
as a loss function for learning CBM.
As a benchmark data set, we used a1a dataset~\cite{a1a},
which has 32,561 records and 123 attributes.
We conduced learning CBM with $C=0.1, 1$ and $k=1,2,3,4,5,6,\infty$.  
%for the respective algorithms.
The results on computation time are shown in Table~\ref{tab:time}.

\begin{table*}[htbp]
\caption{
Comparison of computation time (sec) on a1a dataset:
the bracketed values at \textit{Expand+$L_1$-regularized Logistic Regression}
mean the elapsed times to solve $L_1$-regularized logistic regression.
}
\label{tab:time}
\begin{center}
\begin{tabular}{|r||r|r|r|r|r|r|} \hline
           & \multicolumn{2}{|c|}{GRAB} & \multicolumn{2}{|c|}{Grafting + na\"{i}ve feature selection} & \multicolumn{2}{|c|}{Expansion + $L_1$-regularized Logistic Regression} \\ \hline
           & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$}  & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} \\ \hline
$k=1$      & 2.1 & 1.7 & \ \ \ \ \ \ \ \ \ \ 5.3 & 4.0 & 3.0E-1\ (1.4E-1) & 2.4E-2\ (8.5E-2) \\ \hline
$k=2$      & 4.5 & 5.8E+1 & 3.2E+2 & 2.9E+2 & 3.8\ (3.0E-1) & 3.8\ (3.2E-1) \\ \hline
$k=3$      & 8.7 & 2.1E+1 & 1.3E+4 & 1.2E+4 & 5.5E+1\ (9.8E-1) & 5.5E+1\ (1.1) \\ \hline
$k=4$      & 1.3E+1 & 4.1E+1 & >1 day        & >1 day        & 4.7E+2\ (1.4) & 4.7E+2\ (1.9) \\ \hline
$k=5$      & 1.5E+1 & 9.2E+1 & >1 day        & >1 day        & 2.3E+3\ (5.1) & 2.3E+3\ (5.2) \\ \hline
$k=6$      & 1.7E+1 & 1.4E+2 & >1 day        & >1 day        & 7.6E+3\ (1.3E+1) & 7.6E+3\ (1.1E+1) \\ \hline
$k=\infty$ & 2.3E+1 & 2.9E+2 & >1 day        & >1 day        & 5.6E+4\ (9.2E+1) & 5.6E+4\ (9.1E+1) \\ \hline
\end{tabular}
\end{center}
\end{table*}


We first observe that the computation time for GRAB is significantly smaller than that of of Grafting+Na\"{\i}ve feature selection.
It implies that WFIM was so efficient that it could  select the feature~$\phi\in\Phi^{(k)}$.

%We then compare GRAB with Expansion+$L_1$-regularized logistic regression to have the following observation:
$L_1$-regularized logistic regression solved the parameter optimization problem more quickly than GRAB. 
However, the expansion step took much longer time than the whole procedure of GRAB.
It implies that GRAB learned CBM more efficiently than Expansion+$L_1$-regularized logistic regression.


\subsection{Evaluation of prediction accuracy}

In order to evaluate GRAB's prediction performance,
we conducted experiments for the following benchmark datasets:
\begin{enumerate}
\item
\textbf{a1a}~\cite{a1a}: It has 32,561 records and 123 attributes for each data.
This dataset is obtained by preprocessing  Adult dataset~\cite{Adult},
which has 6 continuous and 8 categorical features.
We divided the total data into 30,000 training data and 2,561 test data.
\item
\textbf{cod-rna}~\cite{cod-rna}:
It is a dataset for the problem of detecting non-coding RNAs from attributes of base sequences.
Since all of  the 8 attributes are real-valued,
we transformed  each attribute into a binary one as follows:
We divided the interval from the minimum value to the maximum value into 30 cells of equal length.
We expressed each attribute in a binary form by indicating which section its value fell into.
Thus, a binary dataset with 240 attributes was obtained.
Each data in it was specified by  8 non-zero attributes.
We used 300,000 data for training and 31,152 for test.
\item
\textbf{covtype.binary}~\cite{covtype.binary}:
It is a dataset obtained by transforming Covertype dataset~\cite{}
with multi labels into the one with binary labels.
The original Covertype dataset has 581,012 instances with 54 cartographic attributes,
and 10 of which are quantitative ones and the rest are binary.
\if 0
and forest cover type categorized by seven as labels.
\fi
We binarized all the quantitative attributes in the same way as cod-rna dataset.
We used 500,000 data for training and 81,012 for test.
\if 0
\item
\textbf{traffic}: was collected from 1,727 intersections in Tokyo,
873 of which are dangerous road points where more than 4 traffic accidents occurred at 2012 (positive example),
and the rest are other non-risky road points (negative example).
At each target intersection, we collect binary of categorical features such as signal type and presence of sidewalks from all the connected road.
For example, when road feature vector
Our task is to predict whether road points are risky or not
from information of intersection structures, such as signal types, presence of sidewalks and so on.
\fi
\end{enumerate}

As methods for comparison, we employed {\em support vector classification} (SVC)
with two types of kernel functions: polynomial kernel (Poly) %(\textit{poly}) 
and radial basis function kernel (RBF), % (\textit{rbf}),
both of which have extensively been used for the purpose of classification.
The polynomial kernel is defined as $k(\bm{x},\bm{x}')=\rbr{\gamma \bm{x}^\top\bm{x}'+\rbr{1-\gamma}}^d$,
where $d\in\mathbb{N}_+$ and $\gamma\in (0,1]$ are hyper parameters,
and radial basis function kernel is defined as $k(\bm{x},\bm{x}')=\exp\rbr{\frac{1}{2\gamma}\|\bm{x}-\bm{x}'\|^2_2}$,
where $\gamma>0$ is a hyper parameter.


We employed the logistic loss  and the $L_2$-hinge loss as loss functions for learning CBM.
The $L_2$-hinge loss function is defined as:
\begin{align*}
\ell(f(\bm{x}), y)\triangleq \begin{cases}
\rbr{1-yf(\bm{x})}^2 & {\rm if}\ 1-yf(\bm{x})<0 ,\\
0 & \text{otherwise.}
\end{cases}
\end{align*}
Note that the WFIM procedure in GRAB can be accelerated
by using the $L_2$-hinge loss.
This is because $\partial \ell(\bm{x}_i,y_i)/\partial f^{(k)}(\bm{x})$,
which is the $i$-th transaction weight of WFIM,
is $0$ for all $i$ satisfying $1-y_if(\bm{x}_i)\geq 0$
and we can remove the corresponding data from the transaction database.

For each of the benchmark datasets,
we compared prediction accuracies of the following algorithms:
\begin{enumerate}
\item Polynomial kernel SVC with $d=1$ and $3$,
\item RBF kernel SVC,
\item Logistic loss CBM with $k=1,3$ and $\infty$, 
\item $L_2$-hinge loss CBM with $k=1,3$ and $\infty$.
\end{enumerate}
For each of the algorithms,  
after learning models with $C=10^{-3},$ $10^{-2},$$\ldots,$ $10^3$ for CBM
and with $\gamma=0.1,0.2,\ldots,1$ for SVC from training data,
we selected the model with the highest accuracy on test data.
%as the final output.


Table~\ref{tab:accuracy} shows the accuracies of the respective algorithms.
From the results on a1a dataset, we see that GRAB with $k=1$ is 
almost comparable to Poly with $d=1$,
while the former finished training more than 100 times faster than the latter.
%while the time complexity of the former is ***  smaller than the latter.
%などの文がほしい
This implies that linear models are accurate enough for the prediction with a1a dataset.
The time complexity of logistic loss GRAB with $k=3$ 
was more than 10 times higher than polynomial kernel SVC with $d=3$.

From the results on cod-rna dataset shown in Table~\ref{tab:accuracy}\subref{tab:accuracy_cod-rna}, 
we observe that the accuracies of SVC on the binarized dataset are much greater than those on the raw one.
The reason for this may be that
cod-rna dataset becomes almost linearly separable by means of binarization.
$L_2$-hinge loss GRAB with  $k=\infty$ is more than $1\%$ more accurate than that with $k=1$. 
This implies that combinatorial features are effective for the prediction with cod-rna dataset.
Poly with $d=3$ on the binarized data, which achieved the highest accuracy among the SVC family, was almost comparable to $L_2$-hinge loss GRAB with $k=\infty$, 
which achieved the  highest accuracy among GRAB family.
However, the computation time of the best in GRABs was less than one hundredth of that of the best in SVCs.
This is because binarized cod-rna dataset was of high sparsity in the sense that the number of nonzero elements per record was just eight out of 240,
and WFIM was  executed very rapidly.


From the results on covtype.binary dataset shown in  Table~\ref{tab:accuracy}\subref{tab:accuracy_covtype.binary}, 
we see that  binarization contributed to the improvement of  accuracies of SVCs.
This was similar to the case of cod-rna.
We also see that combinatorial features greatly contributed to the prediction with covtype.binary dataset.
%計算量の比較も結果がでたら上の要領で書くべし

\begin{table*}[htbp]
\caption{
Comparison of accuracy (\%) on benchmark datasets:
the terms \textit{Raw} and \textit{Binarized} mean that
we used the original and the binarized dataset, respectively,
as a training data.
The row \textit{Time} shows the elapsed time (sec) of each method
when the number of training data is the maximum.
}
\label{tab:accuracy}
\begin{center}
\subfloat[a1a \label{tab:accuracy_a1a}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|} \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
7,500 & 85.2 & 85.3 & 85.2 & 84.9 & 84.7 & 84.9 & 84.9 & 85.3 & 84.5 \\ \hline
30,000 & 85.4 & 85.3 & 85.2 & 85.0 & 85.5 & 85.5 & 85.1 & 85.5 & 84.3 \\ \hline\hline
Time (sec) & 2.3E+2 & 1.0E+2 & 1.4E+2 & 1.4 & 6.9 & 1.7E+1 & 1.2 & 1.4E+1 & 5.0 \\ \hline
\end{tabular}
}

\subfloat[cod-rna \label{tab:accuracy_cod-rna}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 88.9 & 88.8 & 89.3 & 95.6 & 96.0 & 96.0 & 95.5 & 95.9 & 95.9 & 95.5 & 96.0 & 96.0 \\ \hline
100,000 & 89.0 & 88.9 & 90.1 & 95.7 & 96.3 & 96.3 & 95.6 & 96.0 & 96.0 & 95.6 & 96.3 & 96.3 \\ \hline
300,000 & 89.4 & 89.0 & 93.0 & 95.7 & 96.6 & 96.4 & 95.6 & 96.5 & 96.5 & 95.6 & 96.6 & 96.7 \\ \hline\hline
Time (sec) & 3.0E+3 & 3.8E+3 & 5.3E+3 & 8.0E+3 & 1.4E+4 & 1.1E+4 & 6.4E+1 & 2.1E+2 & 1.1E+2 & 1.5E+1 & 8.8E+1 & 1.1E+2 \\ \hline
\end{tabular}
}

\subfloat[covtype.binary \label{tab:accuracy_covtype.binary}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 76.0 & 82.0 & 86.1 & 74.4 & 86.8 & 87.6 & 76.9 & 86.7 & 86.9 & 76.9 & 86.5 & 86.6 \\ \hline
100,000 & 76.1 & 82.4 & 87.0 & 74.1 & 90.6 & 91.2 & 77.0 & 90.8 & 90.9 & 77.0 & 90.4 & 90.6 \\ \hline
500,000 & & & & - & - & - & 76.9 & 94.1 & 94.3 & 77.0 & 94.3 & 94.7 \\ \hline\hline
Time (sec) & & & & > 1 day & > 1 day & > 1 day & 6.6E+1 & 3.7E+3 & 4.7E+3 & 3.8E+1 & 2.6E+3 & 3.6E+3 \\ \hline
\end{tabular}
}
\end{center}
\end{table*}

\subsection{Evaluation of interpretability}
We evaluate interpretability of GRAB.
We can conduct knowledge acquisition from the learning results for GRAB as follows:
Look at the predictor learned by GRAB.
In it the features whose corresponding weights have large absolute values can be interpreted as important ones.
This is because such features greatly affect the prediction results.
Hence, by simply extracting large-valued features,  we can acquire knowledge about what features are important for prediction.
Specifically, features used in GRAB are very comprehensive since they are represented as conjunctions of attributes.
This implies that GRAB is of high interpretability of the acquired knowledge.

\textcolor{red}{
まず、a1a dataset~\cite{a1a}を用いた実験を行なった。
上で述べた通りa1a datasetはAdult datasetを二値化することで得られたデータである
\footnote{
\textcolor{red}{
In \cite[pp. 56--57]{John98},
it has been described as
"The six continuous attributes were discretized into quintiles, which yielded a total of 123 binary attributes."
However, comparing Adult dataset and a1a dataset, we noticed that the dimension does not much.
そこで、monetary capital gainsとmonetary capital lossesに関する量的変数は二値化されており、
その他の量的変数はquintilesに変換されていると解釈した。
}
}
。
Adult datasetは国勢調査局のデータベース(census bureau database)を元に作られており、
年齢や最終学歴などの特徴からその人物の年収が50K\$以上（正例）か未満（負例）かを予測するタスクのためのデータセットである。
Table~\ref{tab:a1a_knowledge} shows weights with large absolute values,
which were obtained by GRAB with $L_2$-hinge loss and $k=3$ on a1a dataset.
まず、1,2番目に絶対値が大きい特徴に注目する。
(Not in family)という特徴はWeightが負であるので、この性質を有することにより負例方向にゲインを得る。
しかしながら、2番目の特徴を見ると(Not in family)の性質を有していても(No monetary capital losses)の性質を有していれば、
逆に正例方向にゲインを得ることがわかる。
また、6番目の特徴からeducation numberが大きいという性質は基本的には正例方向のゲインを与えることがわかる。
しかしながら、興味深いことに、職業が(Other service)であり、労働時間が(Middle average hours per week worked)である時は負例方向のゲインを得るが、
職業が(Prof specialty)であり、(Have monetary capital gains)の時は反対に正例方向のゲインを得ることができる。
このように特徴の組合わせを考慮することにより、粒度の細かい知識発見を行うことができる。
}

\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from a1a dataset.
}
\label{tab:a1a_knowledge}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
-0.581 & (Not in family) \\ \hline
0.544 & (Not in family) \& (No monetary capital losses) \\ \hline
0.455 & (Self-employment (not inc.)) \& (Unmarried) \& (Have monetary capital gains) \\ \hline
-0.432 & (Female) \& (No monetary capital gains) \& (No monetary capital losses) \\ \hline
0.390 & (Low final weight) \& (Asian Pacific Islander) \& (From Japan) \\ \hline
0.353 & (Large education number) \\ \hline
0.325 & (Married AF spouse) \& (No monetary capital gains) \& (From United States) \\ \hline
0.320 & (Married civ spouse) \& (No monetary capital losses) \& (From Canada) \\ \hline
-0.291 & (Large education number) \& (Other service) \& (Middle average hours per week worked) \\ \hline
0.272 & (Slightly larger education number) \& (Prof specialty) \& (Have monetary capital gains) \\ \hline
\end{tabular}
\end{table*}

\textcolor{red}{
続いてcovtype.binaryデータセットから知識発見を行う。
covtype.binary datasetはCovertype datasetをmulti labelからbinary labelに変換することで作成された。
各レコードはRoosevelt National Forest内の4つの荒野区域における30メートル四方のセルに対応している。
Covertype datasetはその地点での標高や勾配、どの荒野区域に所属しているかなどの情報から、
その地点のForest cover typeを7種類の中から予測するタスクのためのデータセットである。
covtype.binary datasetは7種類のForest cover typeのうちタイプ2を正例、その他を負例にすることで
二値分類問題化を行なったものである。
a1aデータセットと異なり、covtype.binaryデータセットはその特徴量に連続値が含まれるため、
前節で述べた通り前処理を行い二値化を施した。
そのため、a1aデータセットの時のようにただ重みの絶対値が大きいものを観察するだけでは、
知見を得ることは困難である。
そこで、次のような学習結果の可視化を提案する。
まず、a1aデータセットの時と同様に重みの絶対値が大きいものを観察した結果、
ElevationとWilderness area designationを組合せた特徴量が大きな絶対値を有することが確認された。
Elevationは連続量、Wilderness area designationはカテゴリカルな量である。
縦軸にElevationを横軸にWilderness area designationの各カテゴリを取り、
全ての組合せについて学習後の重みをプロットしたものを図~\ref{fig:cov_knowledge}(a)に示す。
このプロットを観察することで、組合せた連続量の変化によって予測への寄与がどう変動するかを
視覚的に理解することが可能になる。
図~\ref{fig:cov_knowledge}(a)より、Wilderness area designationの各カテゴリ毎に、
Elevationの振る舞いが異なっていることが確認できる。
特にRawahとComanche Peak間の違いが顕著であり、RawahではElevationが10程度でピークをとり、
それより上に行くほど重みが減少しているのに対し、
Comanche PeakではElevationが15から20程度の間で正の重みを持ち、それより低い場所では負の重みを持っていることが確認できる。
この傾向は線形な学習モデルでは表現することが不可能である。
実際に学習データをElevationとWilderness area designationごとに分類し、正例の割合をプロットしたグラフを
図~\ref{fig:cov_knowledge}(b)に示す。
図~\ref{fig:cov_knowledge}(a)と(b)を比較すると、(a)で赤または青になっている領域は(b)でも同色になっており、
学習データと同様の振る舞いを見せていることが確認できる。
一方で、例えばNeotaとComanche PeakでのElevationが高い部分については、(b)においては青い領域になっているが、
(a)においては重みが0になっていることがわかる。
これは、この領域が他の特徴量によってフィッティングされるべき部分であることを示唆しており、
逆に言うと(a)が(b)と同様の振る舞いを示している領域においては、ElevationとWilderness area designationの組合せ
が有用な知見になっていることを示している。
}

\begin{figure*}[t]
\begin{center}
\subfloat[]{
\includegraphics[width=\columnwidth]{weights.png}
}
\subfloat[]{
\includegraphics[width=\columnwidth]{dist.png}
}
\end{center}    
\caption{
各ElevationとWilderness area designationに対応する組合わせ特徴量の重み(a)と
正例の割合(b)：
}
\label{fig:cov_knowledge}
\end{figure*}

\if 0
\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from covtype.binary dataset.
}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
1.997469 & Elevation(10) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
1.932653 & Elevation(11) \& Horizontal Distance to nearest wildfire ignition point(30) \\ \hline
1.904661 & Elevation(18) \& Horizontal Distance to nearest roadway(17) \& Horizontal Distance to nearest wildfire ignition points(9) \\ \hline
1.887015 & Horizontal Distance to nearest roadway(12) \& Horizontal Distance to nearest wildfire ignition pints(11) \& Leighcan family, till substratum - Typic Cryaquolls complex. \\ \hline
1.810542 & Horizontal Distance to nearest roadway(9) \& Horizontal Distance to nearest wildfire ignition point(278) \& Rawah Wilderness Area(301) \\ \hline
1.775597 & Horizontal Distance to nearest wildfire ignition points(12) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.715680 & Horizontal Distance to nearest wildfire ignition points(11) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.636024 & Elevation(9) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
-1.627047 & Comanche Peak Wilderness Area \\ \hline
1.609355 & Elevation(20) \& Horizontal Distance(7) \& Horizontal Distance to nearest wildfire ignition points(6) \\ \hline
1.601753 & Elevation(11) \\ \hline
1.600297 & Elevation(7) \& Horizontal Distance to nearest roadway(2) \& Horizontal Distance to nearest wildfire ignition points(275) \\ \hline
1.571094 & Elevation(13) \\ \hline
1.565210 & Horizontal Distance to nearest roadway(13) \& Horizontal Distance to nearest wildfire ignition points(13) \& Neota Wilderness Area \\ \hline
\end{tabular}
\end{table*}
\fi

%polymonial kernel is difficult to hyper-tune


==> experiments_0218_2.tex <==
\section{Experiments}
\label{sec:experiments}

We implemented our algorithm GRAB
\footnote{All of our experimental codes are available at 
\url{https://www.dropbox.com/sh/fjjmwkiwt509368/AABR7L2at0vQc4xMld6_WCGoa?dl=0}.}
\textcolor{red}{in C and C++}
to 
evaluate its computational complexity, prediction accuracy, and knowledge interpretability.
In order to select new features to be added, we used Linear time Closed itemset Miner (LCM) by ~\cite{Uno03,Uno04,Uno05}, which is one of backtracking-based FIM  algorithms. All experiments below are executed by Linux (CentOS 6.4) machines 
with 94GB memory and Intel(R) Xeon(R) Processor X5690 @ 3.47GHz.

\subsection{Evaluation of Computation Time}
In order to evaluate the computational efficiency of GRAB, 
we employed benchmark datasets to compare GRAB with other methods.
% in terms of  computation time required for learning CBM.
We investigated how effective the grafting algorithm and WFIM were respectively.
To this end, as methods for comparison, we employed the following two combinations:
\begin{enumerate}
\item{{\em Expansion + $L_1$-regularized logistic regression:}\\}
In this combination, we first expand a dataset so that  all possible features are employed to express $\phi\in\Phi^{(k)}$ ({\em expansion}).
We then learn combinatorial linear models on the expanded data set within the $L_1$-regularized logistic regression framework.
\item{{\em Grafting + Na\"{\i}ve feature selection:}\\}
In this combination we employ the grating algorithm, without combing it with WFIM. 
In it we calculate \eqref{eq:grafting_weight_choice} by searching exhaustively over  the set of all features~$\phi\in\Phi^{(k)}$.
\end{enumerate}

In our experiment, we used the logistic loss function $\ell(f(\bm{x}), y)\triangleq -\log\rbr{1/\rbr{1+\exp\rbr{-yf(\bm{x}}}}$ 
as a loss function for learning CBM.
As a benchmark data set, we used a1a dataset~\cite{Platt99},
which has 32,561 records and 123 attributes.
We conducted learning CBM with $C=0.1, 1$ and $k=1,2,3,4,5,6,\infty$.  
%for the respective algorithms.
The results on computation time are shown in Table~\ref{tab:time}.

\begin{table*}[htbp]
\caption{
Comparison of computation time (sec) on a1a dataset:
the bracketed values at \textit{Expand+$L_1$-regularized Logistic Regression}
mean the elapsed times to solve $L_1$-regularized logistic regression.
}
\label{tab:time}
\begin{center}
\begin{tabular}{|r||r|r|r|r|r|r|} \hline
           & \multicolumn{2}{|c|}{GRAB} & \multicolumn{2}{|c|}{Grafting + Na\"{i}ve feature selection} & \multicolumn{2}{|c|}{Expansion + $L_1$-regularized Logistic Regression} \\ \hline
           & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$}  & \multicolumn{1}{|c|}{$C=1$} & \multicolumn{1}{|c|}{$C=0.1$} & \multicolumn{1}{|c|}{$C=1$} \\ \hline
$k=1$      & 2.1 & 1.7 & \ \ \ \ \ \ \ \ \ \ 5.3 & 4.0 & 3.0E-1\ (1.4E-1) & 2.4E-2\ (8.5E-2) \\ \hline
$k=2$      & 4.5 & 5.8E+1 & 3.2E+2 & 2.9E+2 & 3.8\ (3.0E-1) & 3.8\ (3.2E-1) \\ \hline
$k=3$      & 8.7 & 2.1E+1 & 1.3E+4 & 1.2E+4 & 5.5E+1\ (9.8E-1) & 5.5E+1\ (1.1) \\ \hline
$k=4$      & 1.3E+1 & 4.1E+1 & >1 day        & >1 day        & 4.7E+2\ (1.4) & 4.7E+2\ (1.9) \\ \hline
$k=5$      & 1.5E+1 & 9.2E+1 & >1 day        & >1 day        & 2.3E+3\ (5.1) & 2.3E+3\ (5.2) \\ \hline
$k=6$      & 1.7E+1 & 1.4E+2 & >1 day        & >1 day        & 7.6E+3\ (1.3E+1) & 7.6E+3\ (1.1E+1) \\ \hline
$k=\infty$ & 2.3E+1 & 2.9E+2 & >1 day        & >1 day        & 5.6E+4\ (9.2E+1) & 5.6E+4\ (9.1E+1) \\ \hline
\end{tabular}
\end{center}
\end{table*}


We first observe that the computation time for GRAB is significantly smaller than that of of Grafting+Na\"{\i}ve feature selection.
It implies that WFIM was so efficient that it could  select the feature~$\phi\in\Phi^{(k)}$.

%We then compare GRAB with Expansion+$L_1$-regularized logistic regression to have the following observation:
$L_1$-regularized logistic regression solved the parameter optimization problem more quickly than GRAB. 
However, the expansion step took much longer time than the whole procedure of GRAB.
It implies that GRAB learned CBM more efficiently than Expansion+$L_1$-regularized logistic regression.


\subsection{Evaluation of prediction accuracy}

In order to evaluate GRAB's prediction performance,
we conducted experiments for the following benchmark datasets:
\begin{enumerate}
\item
\textbf{a1a}\footnotemark[1]~\cite{Platt99}: It has 32,561 records and 123 attributes for each data.
This dataset is obtained by preprocessing UCI Adult dataset~\cite{UCI},
which has 6 continuous and 8 categorical features.
We divided the total data into 30,000 training data and 2,561 test data.
\item
\textbf{cod-rna}\footnotemark[1]~\cite{Uzilov06}:
It is a dataset for the problem of detecting non-coding RNAs from attributes of base sequences.
Since all of  the 8 attributes are real-valued,
we transformed  each attribute into a binary one as follows:
We divided the interval from the minimum value to the maximum value into 30 cells of equal length.
We expressed each attribute in a binary form by indicating which section its value fell into.
Thus, a binary dataset with 240 attributes was obtained.
Each data in it was specified by  8 non-zero attributes.
We used 300,000 data for training and 31,152 for test.
\item
\textbf{covtype.binary}\footnotemark[1]~\cite{Collobert02}:
It is a dataset obtained by transforming UCI Covertype dataset~\cite{UCI}
with multi labels into the one with binary labels.
The original Covertype dataset has 581,012 instances with 54 cartographic attributes,
and 10 of which are quantitative ones and the rest are binary.
We binarized all the quantitative attributes in the same way as cod-rna dataset.
We used 500,000 data for training and 81,012 for test.
\end{enumerate}
\footnotetext[1]{
Datasets are available on the LIBSVM Data website at
https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/binary.html.
}

As methods for comparison, we employed {\em support vector classification} (SVC)
with two types of kernel functions: polynomial kernel (Poly) %(\textit{poly}) 
and radial basis function kernel (RBF), % (\textit{rbf}),
both of which have extensively been used for the purpose of classification.
The polynomial kernel is defined as $k(\bm{x},\bm{x}')=\rbr{\gamma \bm{x}^\top\bm{x}'+\rbr{1-\gamma}}^d$,
where $d\in\mathbb{N}_+$ and $\gamma\in (0,1]$ are hyper parameters,
and radial basis function kernel is defined as $k(\bm{x},\bm{x}')=\exp\rbr{\frac{1}{2\gamma}\|\bm{x}-\bm{x}'\|^2_2}$,
where $\gamma>0$ is a hyper parameter.

We employed the logistic loss  and the $L_2$-hinge loss as loss functions for learning CBM.
The $L_2$-hinge loss function is defined as:
\begin{align*}
\ell(f(\bm{x}), y)\triangleq \begin{cases}
\rbr{1-yf(\bm{x})}^2 & {\rm if}\ 1-yf(\bm{x})>0 ,\\
0 & \text{otherwise.}
\end{cases}
\end{align*}
Note that the WFIM procedure in GRAB can be accelerated
by using the $L_2$-hinge loss.
This is because $\partial \ell(\bm{x}_i,y_i)/\partial f^{(k)}(\bm{x})$,
which is the $i$-th transaction weight of WFIM,
is $0$ for all $i$ satisfying $1-y_if(\bm{x}_i)\leq 0$
and we can remove the corresponding data from the transaction database.

For each of the benchmark datasets,
we compared prediction accuracies of the following algorithms:
\begin{enumerate}
\item Polynomial kernel SVC with $d=1$ and $3$,
\item RBF kernel SVC,
\item Logistic loss GRAB with $k=1,3$ and $\infty$, 
\item $L_2$-hinge loss GRAB with $k=1,3$ and $\infty$.
\end{enumerate}
For each of the algorithms,  
after learning models with $C=10^{-3},$ $10^{-2},$$\ldots,$ $10^3$ for GRAB
and with $C=10^{-3},$ $10^{-2},$$\ldots,$ $10^3$ and $\gamma=0.1,0.2,\ldots,1$ for SVC from training data,
we selected the model with the highest accuracy on test data.
\textcolor{red}{
In order to conduct SVCs,
we made use of scikit-learn~\cite{sklearn}, which is a machine learning library written in Python.
Note that it is not unfair to compare computation times of GRAB and SVC,
since the implementation of SVC in sckit-learn is based on LIBSVM~\cite{LIBSVM},
which is written in C and C++.
}


Table~\ref{tab:accuracy} shows the accuracies of the respective algorithms.
From the results on a1a dataset, we see that GRAB with $k=1$ is 
almost comparable to Poly with $d=1$,
while the former finished training more than 100 times faster than the latter.
%while the time complexity of the former is ***  smaller than the latter.
%などの文がほしい
This implies that linear models are accurate enough for the prediction with a1a dataset.
The time complexity of logistic loss GRAB with $k=3$ 
was more than 10 times higher than polynomial kernel SVC with $d=3$.

From the results on cod-rna dataset shown in Table~\ref{tab:accuracy}\subref{tab:accuracy_cod-rna}, 
we observe that the accuracies of SVC on the binarized dataset are much greater than those on the raw one.
The reason for this may be that
cod-rna dataset becomes almost linearly separable by means of binarization.
$L_2$-hinge loss GRAB with  $k=\infty$ is more than $1\%$ more accurate than that with $k=1$. 
This implies that combinatorial features are effective for the prediction with cod-rna dataset.
Poly with $d=3$ on the binarized data, which achieved the highest accuracy among the SVC family, was almost comparable to $L_2$-hinge loss GRAB with $k=\infty$, 
which achieved the  highest accuracy among GRAB family.
However, the computation time of the best in GRABs was less than one hundredth of that of the best in SVCs.
This is because binarized cod-rna dataset was of high sparsity in the sense that the number of nonzero elements per record was just eight out of 240,
and WFIM was  executed very rapidly.


From the results on covtype.binary dataset shown in  Table~\ref{tab:accuracy}\subref{tab:accuracy_covtype.binary}, 
we see that  binarization contributed to the improvement of  accuracies of SVCs.
This was similar to the case of cod-rna.
We also see that combinatorial features greatly contributed to the prediction with covtype.binary dataset.
%計算量の比較も結果がでたら上の要領で書くべし

\begin{table*}[htbp]
\caption{
Comparison of accuracy (\%) on benchmark datasets:
the terms \textit{Raw} and \textit{Binarized} mean that
we used the original and the binarized dataset, respectively,
as a training data.
The row \textit{Time} shows the elapsed time (sec) of each method
when the number of training data is the maximum.
}
\label{tab:accuracy}
\begin{center}
\subfloat[a1a \label{tab:accuracy_a1a}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|} \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
7,500 & 85.2 & 85.3 & 85.2 & 84.9 & 84.7 & 84.9 & 84.9 & 85.3 & 84.5 \\ \hline
30,000 & 85.4 & 85.3 & 85.2 & 85.0 & 85.5 & 85.5 & 85.1 & 85.5 & 84.3 \\ \hline\hline
Time (sec) & 2.3E+2 & 1.0E+2 & 1.4E+2 & 1.4 & 6.9 & 1.7E+1 & 1.2 & 1.4E+1 & 5.0 \\ \hline
\end{tabular}
}

\subfloat[cod-rna \label{tab:accuracy_cod-rna}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 88.9 & 88.8 & 89.3 & 95.6 & 96.0 & 96.0 & 95.5 & 95.9 & 95.9 & 95.5 & 96.0 & 96.0 \\ \hline
100,000 & 89.0 & 88.9 & 90.1 & 95.7 & 96.3 & 96.3 & 95.6 & 96.0 & 96.0 & 95.6 & 96.3 & 96.3 \\ \hline
300,000 & 89.4 & 89.0 & 93.0 & 95.7 & 96.6 & 96.4 & 95.6 & 96.5 & 96.5 & 95.6 & 96.6 & 96.7 \\ \hline\hline
Time (sec) & 3.0E+3 & 3.8E+3 & 5.3E+3 & 8.0E+3 & 1.4E+4 & 1.1E+4 & 6.4E+1 & 2.1E+2 & 1.1E+2 & 1.5E+1 & 8.8E+1 & 1.1E+2 \\ \hline
\end{tabular}
}

\subfloat[covtype.binary \label{tab:accuracy_covtype.binary}]{
\begin{tabular}{|r||r|r|r|r|r|r|r|r|r|r|r|r|} \hline
Dataset & \multicolumn{3}{|c|}{Raw} & \multicolumn{9}{|c|}{Binarized} \\ \hline
 & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{2}{|c|}{Poly} & \multicolumn{1}{|c|}{RBF} & \multicolumn{3}{|c|}{GRAB (logistic loss)} & \multicolumn{3}{|c|}{GRAB ($L_2$-hinge loss)} \\ \hline
\#Data & $d=1$ & $d=3$ & & $d=1$ & $d=3$ & & $k=1$ & $k=3$ & $k=\infty$ & $k=1$ & $k=3$ & $k=\infty$ \\ \hline
50,000 & 76.0 & 82.0 & 86.1 & 74.4 & 86.8 & 87.6 & 76.9 & 86.7 & 86.9 & 76.9 & 86.5 & 86.6 \\ \hline
100,000 & 76.1 & 82.4 & 87.0 & 74.1 & 90.6 & 91.2 & 77.0 & 90.8 & 90.9 & 77.0 & 90.4 & 90.6 \\ \hline
500,000 & & & & - & - & - & 76.9 & 94.1 & 94.3 & 77.0 & 94.3 & 94.7 \\ \hline\hline
Time (sec) & & & & > 1 day & > 1 day & > 1 day & 6.6E+1 & 3.7E+3 & 4.7E+3 & 3.8E+1 & 2.6E+3 & 3.6E+3 \\ \hline
\end{tabular}
}
\end{center}
\end{table*}

\subsection{Evaluation of interpretability}
We evaluate interpretability of GRAB.
We can conduct knowledge acquisition from the learning results for GRAB as follows:
Look at the predictor learned by GRAB.
In it the features whose corresponding weights have large absolute values can be interpreted as important ones.
This is because such features greatly affect the prediction results.
Hence, by simply extracting large-valued features,  we can acquire knowledge about what features are important for prediction.
Specifically, features used in GRAB are very comprehensive since they are represented as conjunctions of attributes.
This implies that GRAB is of high interpretability of the acquired knowledge.

Below we show the results on knowledge discovery for a1a dataset~\cite{Platt99}.
%を用いた実験を行なった。
%上で述べた通りa1a datasetはAdult datasetを二値化することで得られたデータである
%\footnote{
%\textcolor{red}{
%In \cite[pp. 56--57]{John98},
%it has been described as
%"The six continuous attributes were discretized into quintiles, which yielded a total of 123 binary attributes."
%However, comparing Adult dataset and a1a dataset, we noticed that the dimension does not much.
%そこで、monetary capital gainsとmonetary capital lossesに関する量的変数は二値化されており、
%その他の量的変数はquintilesに変換されていると解釈した。
%}
%}
This dataset was obtained by binarizing the adult dataset, which was extracted from 
the census bureau database
The a1a data set has been used as a benchmark for classification of people with more than \$50,000 annual income or the others, on the basis of their attributes.

Table~\ref{tab:a1a_knowledge} shows weights with large absolute values,
which were obtained by GRAB with $L_2$-hinge loss and $k=3$ on a1a dataset.
The features having large absolute values of weight are listed in a descending order.
This list itself is of high intepretability and represents knowledge acquired from the dataset. 

The feature with the largest absolute value of  weight is (Not in family), which has a negative gain for classification.
The feature with the secondly largest absolute value of weight is 
(Not in family)\&(No monetary capital losses), which has a positive gain for classification. 
It is interesting to see that an identical attribute (Not in family) can contribute to both of the positive and negative gains for classification. 
This suggests the importance of conjunctions of attributes in knowledge discovery.

The feature  with the 6-th largest absolute value of weight is 
(large education number), which has a positive gain for classification. 
But its conjunction with (Other service) \& (Middle average hours per week worked) has a negative gain (the 9-th feature) while its conjunction with (Prof specialty)\&(Have monetary capital gains) has a positive gain (the 10-th feature).
Hence making combinations of attributes is really informative for deepening knowledge discovery.

\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from a1a dataset.
}
\label{tab:a1a_knowledge}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
-0.581 & (Not in family) \\ \hline
0.544 & (Not in family) \& (No monetary capital losses) \\ \hline
0.455 & (Self-employment (not inc.)) \& (Unmarried) \& (Have monetary capital gains) \\ \hline
-0.432 & (Female) \& (No monetary capital gains) \& (No monetary capital losses) \\ \hline
0.390 & (Low final weight) \& (Asian Pacific Islander) \& (From Japan) \\ \hline
0.353 & (Large education number) \\ \hline
0.325 & (Married AF spouse) \& (No monetary capital gains) \& (From United States) \\ \hline
0.320 & (Married civ spouse) \& (No monetary capital losses) \& (From Canada) \\ \hline
-0.291 & (Large education number) \& (Other service) \& (Middle average hours per week worked) \\ \hline
0.272 & (Slightly larger education number) \& (Prof specialty) \& (Have monetary capital gains) \\ \hline
\end{tabular}
\end{table*}

\if 0
\textcolor{red}{
続いてcovtype.binaryデータセットから知識発見を行う。
covtype.binary datasetはCovertype datasetをmulti labelからbinary labelに変換することで作成された。
各レコードはRoosevelt National Forest内の4つの荒野区域における30メートル四方のセルに対応している。
Covertype datasetはその地点での標高や勾配、どの荒野区域に所属しているかなどの情報から、
その地点のForest cover typeを7種類の中から予測するタスクのためのデータセットである。
covtype.binary datasetは7種類のForest cover typeのうちタイプ2を正例、その他を負例にすることで
二値分類問題化を行なったものである。
a1aデータセットと異なり、covtype.binaryデータセットはその特徴量に連続値が含まれるため、
前節で述べた通り前処理を行い二値化を施した。
そのため、a1aデータセットの時のようにただ重みの絶対値が大きいものを観察するだけでは、
知見を得ることは困難である。
そこで、次のような学習結果の可視化を提案する。
まず、a1aデータセットの時と同様に重みの絶対値が大きいものを観察した結果、
ElevationとWilderness area designationを組合せた特徴量が大きな絶対値を有することが確認された。
Elevationは連続量、Wilderness area designationはカテゴリカルな量である。
縦軸にElevationを横軸にWilderness area designationの各カテゴリを取り、
全ての組合せについて学習後の重みをプロットしたものを図~\ref{fig:cov_knowledge}(a)に示す。
このプロットを観察することで、組合せた連続量の変化によって予測への寄与がどう変動するかを
視覚的に理解することが可能になる。
図~\ref{fig:cov_knowledge}(a)より、Wilderness area designationの各カテゴリ毎に、
Elevationの振る舞いが異なっていることが確認できる。
特にRawahとComanche Peak間の違いが顕著であり、RawahではElevationが10程度でピークをとり、
それより上に行くほど重みが減少しているのに対し、
Comanche PeakではElevationが15から20程度の間で正の重みを持ち、それより低い場所では負の重みを持っていることが確認できる。
この傾向は線形な学習モデルでは表現することが不可能である。
実際に学習データをElevationとWilderness area designationごとに分類し、正例の割合をプロットしたグラフを
図~\ref{fig:cov_knowledge}(b)に示す。
図~\ref{fig:cov_knowledge}(a)と(b)を比較すると、(a)で赤または青になっている領域は(b)でも同色になっており、
GRABが予測に有用な特徴を適切に選択できていることが確認できる。
}

\begin{figure*}[t]
\begin{center}
\subfloat[]{
\includegraphics[width=\columnwidth]{weights.png}
}
\subfloat[]{
\includegraphics[width=\columnwidth]{dist.png}
}
\end{center}    
\caption{
各ElevationとWilderness area designationに対応する組合わせ特徴量の重み(a)と
正例の割合(b)：
}
\label{fig:cov_knowledge}
\end{figure*}
\fi

\if 0
\begin{table*}
\caption{
Weights with top-10 large absolute values obtained from covtype.binary dataset.
}
\begin{tabular}{|r|c|} \hline
Weight & Combination of Attributes \\ \hline
1.997469 & Elevation(10) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
1.932653 & Elevation(11) \& Horizontal Distance to nearest wildfire ignition point(30) \\ \hline
1.904661 & Elevation(18) \& Horizontal Distance to nearest roadway(17) \& Horizontal Distance to nearest wildfire ignition points(9) \\ \hline
1.887015 & Horizontal Distance to nearest roadway(12) \& Horizontal Distance to nearest wildfire ignition pints(11) \& Leighcan family, till substratum - Typic Cryaquolls complex. \\ \hline
1.810542 & Horizontal Distance to nearest roadway(9) \& Horizontal Distance to nearest wildfire ignition point(278) \& Rawah Wilderness Area(301) \\ \hline
1.775597 & Horizontal Distance to nearest wildfire ignition points(12) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.715680 & Horizontal Distance to nearest wildfire ignition points(11) \& Rawah Wilderness Area \& Leighcan family, till substratum, extremely bouldery. \\ \hline
1.636024 & Elevation(9) \& Horizontal Distance to nearest wildfire ignition points(30) \\ \hline
-1.627047 & Comanche Peak Wilderness Area \\ \hline
1.609355 & Elevation(20) \& Horizontal Distance(7) \& Horizontal Distance to nearest wildfire ignition points(6) \\ \hline
1.601753 & Elevation(11) \\ \hline
1.600297 & Elevation(7) \& Horizontal Distance to nearest roadway(2) \& Horizontal Distance to nearest wildfire ignition points(275) \\ \hline
1.571094 & Elevation(13) \\ \hline
1.565210 & Horizontal Distance to nearest roadway(13) \& Horizontal Distance to nearest wildfire ignition points(13) \& Neota Wilderness Area \\ \hline
\end{tabular}
\end{table*}
\fi

%polymonial kernel is difficult to hyper-tune


==> fim0215.tex <==
\section{Frequent Itemset Mining}
\label{sec:fim}
\begin{figure*}
\begin{center}
\includegraphics[clip,width=18cm]{fim.pdf}
\end{center}
\caption{Demonstration of frequent itemset mining (FIM) and its variants: in the standard setting of FIM, all the transaction are treated homogeneously 
and it searches all itemsets that appears in a given transaction database more than twice (left panel).  Non-negatively weighted FIM (NWFIM)
deal with non-negative weights with respect to each transaction and find itemsets weighted frequency of which is more than 2 (middle panel).
Weighted FIM (WFIM) allows weights on transaction to be negative and loses the monotonicity of output (right panel).}
\end{figure*}
It is difficult in general to find best parameter in terms of grafting algorithm, i.e., 
computing \eqref{eq:grafting_weight_choice} as it requires to compute maximum of 
values corresponding to all components of the parameter.
In this section we review technique for frequent itemset mining, which can cope with this difficulty. 

\subsection*{Terminology}
A set of items $\mathcal{I}=\{1,\ldots,n\}$ is called \emph{item base}.
Also, we call $\mathcal{T}=\{t_1,\ldots,t_m\}$ {\it transaction database},
where each $t_i$ is a subset of $\mathcal{I}$.
We call each element of transaction database {\it a transaction}.

Given a transaction database, an {\it occurence set} of $p\subset \mathcal{I}$, denoted by $\mathcal{T}(p)$,
is a set of all transactions that include $p$, i.e.,  the definition of can be represetned as  
\begin{align}
\mathcal{T}(p) \triangleq \{t\in\mathcal{T}\ |\ t\supseteq p\}.
\end{align}
The cardinality of $\mathcal{T}(p)$ is called frequency and denoted as $\mathrm{frq}(p;\mathcal{T})$:
\begin{align}
\mathrm{frq}(p;\mathcal{T}) \triangleq \sum_{ t \in \mathcal{T}(p)} 1.
\end{align}
By referring to a subset of item base $p$ by an {\it itemset},
The simplest example of frequent itemset mining is a problem to output $\mathcal{P}$, that is, all itemsets with a larger frequency than $\theta$, i.e.,
\begin{align}
\mathcal{P} = \{p\subseteq \mathcal{I}\ |\ \mathrm{frq}(p;\mathcal{T}) > \theta\}
\end{align}
given transaction database $\mathcal{T}$ and threshold $\theta$.

\paragraph{Efficiency}
It is obvious that any subset of an itemset $p$ is included by a transaction $t$ when 
$p$ is included by $t$.
In other words, we can see that a kind of monotonicity holds in such a sense that
\begin{align}
\label{eq:monotonicity}
\mathcal{T}(p')\supseteq\mathcal{T}(p), \ \mathrm{ and } \ \mathrm{frq}(p';\mathcal{T})\geq\mathrm{frq}(p;\mathcal{T}),
\end{align}
for all $p' \subset p$.  
By making use of this property,
we can search all frequent item sets by adding item one by one from $\emptyset$.
Algorithms that performs this search by breadth-first manner are apriori algorithms,
whereas those that perfoms  this search by depth-fast manner are backtracking algorithms.

The size of transaction database, denoted by $\nbr{\mathcal{T}}$, is defined by $\|\mathcal{T}\|  \triangleq \sum_{i=1}^m|t_i|$.
Time complexity of those algorithm are $\mathcal{O}(n\|\mathcal{T}\||\mathcal{P}|)$, which is called output-polynomial time.
Therefore, we can expect that it can run in practical time even when $d$ is large if $|\mathcal{P}|$ is small, 
although  in the worst case that $|\mathcal{P}|$ can be exponentially large.
Apriori algorithm has been firstly proposed by \cite{Agrawal94}.
Frequent item set mining algorithm based on backtraking algorithms are proposed by 
multiple researches, e.g., ~\cite{Zaki97} and~\cite{Bayardo98}.


\subsection*{Weighted FIM}

Standard frequent itemset mining treats transactions as if there are no difference in 
importance among transactions, although, in reality, there often appears such cases
that different importance in each transaction has to be considered.
The values representing importance can be positive and negative, in such cases that, for instance, 
each transaction is allocated to a positive or negative label and one is motivated
to discover itemsets that frequently appears in positive transactions and
not frequently in negative transactions.

In the setting in which only positive has to be dealt with,
we can utilize backtracking algorithm or apriori algorithm and efficient 
algorithm can be constructed, as the monotonicity of frequent itemsets is still maintained.
We define {\it weighted frequency} as follows:
\begin{align}
\mathrm{frq}(p;\mathcal{T},\alpha) \triangleq \sum_{ t \in \mathcal{T}(p)} \alpha_t.
\end{align}
for given $\alpha_t$ for $t\in \mathcal{T}$. 
Even in such cases, we see the same monotonicity as \eqref{eq:monotonicity} still holds and can be 
exploited for non-negativelly-weighted frequent itemset mining,
that is,  tasks to find all itemsets with larger weighted frequency than a given threshold.
However, in the setting in which positive and negative importance has to be dealt with,
the monotonicity of frequent itemset is no longer maintained.
In such cases, algorithms of output-polynomial time are no longer expected to exist, but
the following two-stage strategy is often used and known to be executable for practical usage;
First, we ignore transactions with negative importance and obtain frequent itemset
\begin{align}
\mathcal{P}_+ = \{p\subseteq \mathcal{I}\ |\ \mathrm{frq}(p ; \mathcal{T}_+, \alpha )>\theta\}.
\end{align}
Here positive and negative transactions in $\mathcal{T} $ denoted as $\mathcal{T}_+ $ and $\mathcal{T}_- $ .
Secondly, each itemset in $\mathcal{P}_+$ is checked if desired frequency $\mathrm{frq}(p ; \mathcal{T})$ 
is still larger than $\theta$. The first stage takes a computation 
time $\mathcal{O}(n\|\mathcal{T}_+\||\mathcal{P_+}|)$ by using aforementioned algorithms 
and  second does $\mathcal{O}(n\|\mathcal{T_-}\||\mathcal{P_+}|)$ by accessing all negative transactions for each itemset obtained at 
the first stage. Therefore, in total the computation time required is $\mathcal{O}(n\|\mathcal{T}\||\mathcal{P}_+|)$. 
These three types of frequent itemset mining are demonstrated by examples in Figure~\ref{fig:fim}

\if 0
頻出アイテム集合マイニングはデータマイニングの分野においての最も基本的な問題の一つであり，
アソシエーションルールマイニングなど多くの応用がある．

\paragraph{アプリオリ法}
アプリオリ法はAgrawal and Srikant~\cite{Agrawal94}によって初めて提案された．
アルゴリズム~\ref{algo:apriori}にアプリオリ法を示す．
\begin{algorithm}[!h]
\caption{アプリオリ法}
\label{algo:apriori}
\begin{algorithmic}[1]
\REQUIRE $\theta$：閾値
\STATE $\mathcal{P}_1\leftarrow\text{サイズ1の頻出集合の族}$
\STATE $k\leftarrow 1$
\WHILE {$\mathcal{P}_k\not=\emptyset$}
\STATE $\mathcal{P}_{k+1}\leftarrow(\text{$\mathcal{P}_k$の2つのアイテム集合の和集合でサイズが$k+1$の集合からなる族})$
\STATE $\forall p\in \mathcal{P}_{k+1}, \mathrm{frq}(p)<\theta$を$\mathcal{P}_{k+1}$から取り除く．
\STATE $k\leftarrow k+1$
\ENDWHILE
\STATE \textbf{output} $\mathcal{P}_1,\ldots,\mathcal{P}_{k-1}$
\end{algorithmic}
\end{algorithm}

アプリオリ法の時間計算量について考える．
アプリオリ法のステップ~5における$\mathcal{P}_{k+1}$の各アイテム集合の頻出度の計算に関しては，
アルゴリズム~\ref{algo:calc_freqs}を適用することで，データベースのスキャン1回のみで実行可能である．

\begin{algorithm}[!h]
\caption{頻出度の計算}
\label{algo:calc_freqs}
\begin{algorithmic}[1]
\REQUIRE $\mathcal{T}$：トランザクションデータベース，$\mathcal{P}_{k+1}$：アプリオリ法におけるサイズ~$k+1$の頻出アイテム集合の候補の族
\FORALL {$p\in\mathcal{P}_{k+1}$}
\STATE $\mathrm{frq}(p)\leftarrow 0$
\ENDFOR
\FORALL {$t\in\mathcal{T}$}
\FORALL {$p\in\mathcal{P}_{k+1}$}
\IF {$p\subseteq t$}
\STATE $\mathrm{frq}(p)\leftarrow \mathrm{frq}(p) + 1$
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\paragraph{バックトラック法}
バックトラック法のアルゴリズムを示す前に用語を導入する．
アイテム集合~$X$に対して，$X$中の最大のアイテムを\emph{末尾}（tail）と呼び$\mathrm{tail}(X)$と表す．
ただし$\mathrm{tail}(\emptyset)=-\infty$と定義する．
例えば$\mathrm{tail}(\{1,2,7\})=7$である．
また，アイテム集合~$X$をアイテム集合~$X-\{\mathrm{tail}(X)\}$から生成することを\emph{末尾拡張}（tail extension）と呼ぶ．
例えばアイテム集合~$\{1,2,4,7\}$は$\{1,2,4\}$の末尾拡張である．

末尾拡張を用いてバックトラック法が得られる．
アルゴリズム~\ref{algo:backtracking}にバックトラック法を示す．
バックトラック法は再帰的に定義されており，$\mathrm{Backtracking}(\emptyset)$を計算することで
全ての頻出アイテム集合が出力される．
\begin{algorithm}[!h]
\caption{$\mathrm{Backtracking}(X)$}
\label{algo:backtracking}
\begin{algorithmic}[1]
\REQUIRE $\theta$：閾値
\STATE \textbf{output} $X$
\FORALL {$i>\mathrm{tail}(X)$}
\IF {$\mathrm{frq}(X\cup\{i\})\geq\theta$}
\STATE $\mathrm{Backtracking}(X\cup\{i\})$
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

バックトラック法の時間計算量について考える．
バックトラック法において頻出度~$\mathrm{frq}(\cdot)$の計算は各頻出アイテム集合の末尾拡張の合計回だけ行われる．
またある頻出アイテム集合~$X$に対してその末尾拡張は高々~$n$個であり，1回の頻出度の計算には~$\mathcal{O}(\|\mathcal{T}\|)$
かかるので，合計で$\mathcal{O}(n\|\mathcal{T}\||\mathcal{P}|)$時間でありアプリオリ法と同様となる．
\fi



==> fim_0217.tex <==
\section{Frequent Itemset Mining}
\label{sec:fim}
\begin{figure*}
\begin{center}
\includegraphics[clip,width=2.1\columnwidth]{fim.pdf}
\end{center}
\caption{Demonstration of frequent itemset mining (FIM) and its variants: in the standard setting of FIM, all the transaction are treated homogeneously 
and it searches all itemsets that appears in a given transaction database more than twice (left panel).  Non-negatively weighted FIM (NWFIM)
deal with non-negative weights with respect to each transaction and find itemsets weighted frequency of which is more than 2 (middle panel).
Weighted FIM (WFIM) allows weights on transaction to be negative and loses the monotonicity of output (right panel).}
\end{figure*}
It is computationally difficult to find the best parameter according to \eqref{eq:grafting_weight_choice}. 
This is because  it requires computation of the gradient of loss over 
 all of the components of the parameter.
In order to overcome this difficulty, we employ the technique for frequent itemset mining~(FIM). In this section  we briefly review FIM. 
 

\subsection*{Terminology}
A set of items $\mathcal{I}=\{1,\ldots,n\}$ is called the \emph{item base}.
Also, we call $\mathcal{T}=\{t_1,\ldots,t_m\}$ the {\it transaction database},
where each $t_i$ is a subset of $\mathcal{I}$.
We call each element of  the transaction database {\it a transaction}.

Given a transaction database, an {\it occurrence set} of $p\subset \mathcal{I}$, denoted by $\mathcal{T}(p)$,
is a set of all transactions that include $p$, i.e.,  
\begin{align}
\mathcal{T}(p) \triangleq \{t\in\mathcal{T}\ |\ t\supseteq p\}.
\end{align}
The cardinality of $\mathcal{T}(p)$ is called frequency, which is denoted as $\mathrm{frq}(p;\mathcal{T})$:
\begin{align}
\mathrm{frq}(p;\mathcal{T}) \triangleq \sum_{ t \in \mathcal{T}(p)} 1.
\end{align}
We refer to a subset of item base $p$ as an {\it itemset}.
The simplest example of FIM problem is given as follows: For a given transaction database $\mathcal{T}$ and threshold $\theta$,  find $\mathcal{P}$, which is the set of all itemsets with a larger frequency than $\theta$, i.e.,
\begin{align}
\mathcal{P} = \{p\subseteq \mathcal{I}\ |\ \mathrm{frq}(p;\mathcal{T}) > \theta\}
\end{align}


\subsection{Efficient Algorithms by Utilizing Monotonicity }
It is obvious that any subset of an itemset $p$ is included by a transaction $t$ when 
$p$ is included by $t$.
In other words, we can see that a kind of monotonicity holds in the sense that
\begin{align}
\label{eq:monotonicity}
\mathcal{T}(p')\supseteq\mathcal{T}(p), \ \mathrm{ and } \ \mathrm{frq}(p';\mathcal{T})\geq\mathrm{frq}(p;\mathcal{T}),
\end{align}
for all $p' \subset p$.  
By making use of this property,
we can search all frequent itemsets by adding an item one by one from $\emptyset$.
The algorithm that performs this search in the breadth-first manner is the {\em apriori algorithm},
whereas the one that performs  this search in the depth-fast manner is the {\em backtracking algorithm}.
The apriori algorithm was firstly proposed by \cite{Agrawal94}.
An FIM algorithm based on the backtraking algorithm was proposed in  
e.g., ~\cite{Zaki97} and~\cite{Bayardo98}.

The size of transaction database, denoted as $\nbr{\mathcal{T}}$, is defined by $\|\mathcal{T}\|  \triangleq \sum_{i=1}^m|t_i|$.
Time complexities for both of the apriori and backtracking algorithms are $\mathcal{O}(n\|\mathcal{T}\||\mathcal{P}|)$, which is called the {\em output-polynomial time}.
Hence, they are expected to run in practical time 
as long as $|\mathcal{P}|$ is small
even when $d$ is large, and $|\mathcal{P}|$ is exponentially large in the worst case.

\subsection*{Extension to Weighted FIM}
Standard FIM methods handle transactions as if there were no difference in 
importance among transactions. 
However, there often appear such cases
that importance may differ one another depending on transactions.
Actually, the values of importance may be positive and negative.
If each transaction is allocated to a positive or negative label,
then one may be motivated
to discover itemsets that frequently appear in positive transactions and
not frequently in negative transactions.

In the setting where only the positive importance has to be dealt with,
we can utilize the backtracking algorithm or the apriori algorithm.  
An efficient 
algorithm can be constructed, as the monotonicity of frequent itemsets is still maintained.
We define {\it weighted frequency} as follows:
\begin{align}
\mathrm{frq}(p;\mathcal{T},\alpha) \triangleq \sum_{ t \in \mathcal{T}(p)} \alpha_t.
\end{align}
for given $\alpha_t$ for $t\in \mathcal{T}$.
The same monotonicity as \eqref{eq:monotonicity} still holds for the weighted variant of frequencies.
We are then led to non-negatively-weighted FIM, 
It is to find all itemsets with larger weighted frequency than a given threshold.
However, in the setting where both positive and negative importance has to be dealt with,
the monotonicity of frequent itemset does not hold any longer.
Then any algorithm of output-polynomial time may not exist.
However, we may instead employ the following two-stage strategy:
%It is known to be executable for practical use;
Let the sets of positive and negative transactions in $\mathcal{T} $ be $\mathcal{T}_+ $ and $\mathcal{T}_- $, respectively.
In the first stage, ignoring transactions with negative importance, we obtain frequent itemsets such that 
\begin{align}
\mathcal{P}_+ = \{p\subseteq \mathcal{I}\ |\ \mathrm{frq}(p ; \mathcal{T}_+, \alpha )>\theta\}.
\end{align}
In the second stage,  for each itemset in $\mathcal{P}_+$ we check if a desired frequency $\mathrm{frq}(p ; \mathcal{T})$ 
is still larger than $\theta$. The first stage is executed using 
the aforementioned algorithms in time  $\mathcal{O}(n\|\mathcal{T}_+\||\mathcal{P_+}|)$ 
while the second stage is executed in time
 $\mathcal{O}(n\|\mathcal{T_-}\||\mathcal{P_+}|)$ by accessing all negative transactions for each itemset obtained in 
the first stage. 
Then the total computation time is $\mathcal{O}(n\|\mathcal{T}\||\mathcal{P}_+|)$. 
The three types of FIM as above are illustrated in Figure~\ref{fig:fim}.

\if 0
頻出アイテム集合マイニングはデータマイニングの分野においての最も基本的な問題の一つであり，
アソシエーションルールマイニングなど多くの応用がある．

\paragraph{アプリオリ法}
アプリオリ法はAgrawal and Srikant~\cite{Agrawal94}によって初めて提案された．
アルゴリズム~\ref{algo:apriori}にアプリオリ法を示す．
\begin{algorithm}[!h]
\caption{アプリオリ法}
\label{algo:apriori}
\begin{algorithmic}[1]
\REQUIRE $\theta$：閾値
\STATE $\mathcal{P}_1\leftarrow\text{サイズ1の頻出集合の族}$
\STATE $k\leftarrow 1$
\WHILE {$\mathcal{P}_k\not=\emptyset$}
\STATE $\mathcal{P}_{k+1}\leftarrow(\text{$\mathcal{P}_k$の2つのアイテム集合の和集合でサイズが$k+1$の集合からなる族})$
\STATE $\forall p\in \mathcal{P}_{k+1}, \mathrm{frq}(p)<\theta$を$\mathcal{P}_{k+1}$から取り除く．
\STATE $k\leftarrow k+1$
\ENDWHILE
\STATE \textbf{output} $\mathcal{P}_1,\ldots,\mathcal{P}_{k-1}$
\end{algorithmic}
\end{algorithm}

アプリオリ法の時間計算量について考える．
アプリオリ法のステップ~5における$\mathcal{P}_{k+1}$の各アイテム集合の頻出度の計算に関しては，
アルゴリズム~\ref{algo:calc_freqs}を適用することで，データベースのスキャン1回のみで実行可能である．

\begin{algorithm}[!h]
\caption{頻出度の計算}
\label{algo:calc_freqs}
\begin{algorithmic}[1]
\REQUIRE $\mathcal{T}$：トランザクションデータベース，$\mathcal{P}_{k+1}$：アプリオリ法におけるサイズ~$k+1$の頻出アイテム集合の候補の族
\FORALL {$p\in\mathcal{P}_{k+1}$}
\STATE $\mathrm{frq}(p)\leftarrow 0$
\ENDFOR
\FORALL {$t\in\mathcal{T}$}
\FORALL {$p\in\mathcal{P}_{k+1}$}
\IF {$p\subseteq t$}
\STATE $\mathrm{frq}(p)\leftarrow \mathrm{frq}(p) + 1$
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\paragraph{バックトラック法}
バックトラック法のアルゴリズムを示す前に用語を導入する．
アイテム集合~$X$に対して，$X$中の最大のアイテムを\emph{末尾}（tail）と呼び$\mathrm{tail}(X)$と表す．
ただし$\mathrm{tail}(\emptyset)=-\infty$と定義する．
例えば$\mathrm{tail}(\{1,2,7\})=7$である．
また，アイテム集合~$X$をアイテム集合~$X-\{\mathrm{tail}(X)\}$から生成することを\emph{末尾拡張}（tail extension）と呼ぶ．
例えばアイテム集合~$\{1,2,4,7\}$は$\{1,2,4\}$の末尾拡張である．

末尾拡張を用いてバックトラック法が得られる．
アルゴリズム~\ref{algo:backtracking}にバックトラック法を示す．
バックトラック法は再帰的に定義されており，$\mathrm{Backtracking}(\emptyset)$を計算することで
全ての頻出アイテム集合が出力される．
\begin{algorithm}[!h]
\caption{$\mathrm{Backtracking}(X)$}
\label{algo:backtracking}
\begin{algorithmic}[1]
\REQUIRE $\theta$：閾値
\STATE \textbf{output} $X$
\FORALL {$i>\mathrm{tail}(X)$}
\IF {$\mathrm{frq}(X\cup\{i\})\geq\theta$}
\STATE $\mathrm{Backtracking}(X\cup\{i\})$
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

バックトラック法の時間計算量について考える．
バックトラック法において頻出度~$\mathrm{frq}(\cdot)$の計算は各頻出アイテム集合の末尾拡張の合計回だけ行われる．
またある頻出アイテム集合~$X$に対してその末尾拡張は高々~$n$個であり，1回の頻出度の計算には~$\mathcal{O}(\|\mathcal{T}\|)$
かかるので，合計で$\mathcal{O}(n\|\mathcal{T}\||\mathcal{P}|)$時間でありアプリオリ法と同様となる．
\fi



==> fim_0218.tex <==
\section{Frequent Itemset Mining}
\label{sec:fim}
\begin{figure*}
\begin{center}
\includegraphics[clip,width=2\columnwidth]{fim.pdf}
\end{center}
\caption{Demonstration of frequent itemset mining (FIM) and its variants: in the standard setting of FIM, all the transaction are treated homogeneously 
and it searches all itemsets that appears in a given transaction database more than once (left panel).  Non-negatively weighted FIM (NWFIM)
deal with non-negative weights with respect to each transaction and find itemsets weighted frequency of which is more than 1 (middle panel).
Weighted FIM (WFIM) allows weights on transaction to be negative and loses the monotonicity of output (right panel).}
\label{fig:fim}
\end{figure*}
It is computationally difficult to find the best parameter according to \eqref{eq:grafting_weight_choice}. 
This is because  it requires computation of the gradient of loss over 
 all of the components of the parameter.
In order to overcome this difficulty, we employ the technique for frequent itemset mining~(FIM). In this section  we briefly review FIM. 
 

\subsection*{Terminology}
A set of items $\mathcal{I}=\{1,\ldots,d\}$ is called the \emph{item base}. 
The set $\mathcal{T}=\{t_1,\ldots,t_m\}$ is called the {\it transaction database},
where each $t_i$ is a subset of $\mathcal{I}$.
Each element of  the transaction database  is called {\it a transaction}.

Given a transaction database, an {\it occurrence set} of $p\subset \mathcal{I}$, denoted by $\mathcal{T}(p)$,
is a set of all transactions that include $p$, i.e.,  
\begin{align}
\mathcal{T}(p) \triangleq \{t\in\mathcal{T}\ |\ t\supseteq p\}.
\end{align}
The cardinality of $\mathcal{T}(p)$ is called frequency, which is denoted as $\mathrm{frq}(p;\mathcal{T})$:
\begin{align}
\mathrm{frq}(p;\mathcal{T}) \triangleq \sum_{ t \in \mathcal{T}(p)} 1.
\end{align}
We refer to a subset of item base $p$ as an {\it itemset}.
The simplest example of FIM problem is given as follows: For a given transaction database $\mathcal{T}$ and threshold $\theta$,  find $\mathcal{P}$, which is the set of all itemsets with a larger frequency than $\theta$, i.e.,
\begin{align}
\mathcal{P} = \{p\subseteq \mathcal{I}\ |\ \mathrm{frq}(p;\mathcal{T}) > \theta\}.
\end{align}


\subsection{Efficient Algorithms by Utilizing Monotonicity }
It is obvious that any subset of an itemset $p$ is included by a transaction $t$ when 
$p$ is included by $t$.
In other words, a kind of monotonicity holds in the following sense:
\begin{align}
\label{eq:monotonicity}
\mathcal{T}(p')\supseteq\mathcal{T}(p), \ \mathrm{ and } \ \mathrm{frq}(p';\mathcal{T})\geq\mathrm{frq}(p;\mathcal{T}),
\end{align}
for all $p' \subset p$.  
By making use of this property,
we can search all frequent itemsets by adding an item one by one from $\emptyset$.
The algorithm that performs this search in the breadth-first manner is the {\em apriori algorithm},
whereas the one that performs  this search in the depth-fast manner is the {\em backtracking algorithm}.
The apriori algorithm was firstly proposed by \cite{Agrawal94}.
An FIM algorithm based on the backtraking algorithm was proposed in  
e.g., ~\cite{Zaki97} and~\cite{Bayardo98}.

The size of transaction database, denoted as $\nbr{\mathcal{T}}$, is defined by $\|\mathcal{T}\|  \triangleq \sum_{i=1}^m|t_i|$.
Time complexities for both of the apriori and backtracking algorithms are $\mathcal{O}(m\|\mathcal{T}\||\mathcal{P}|)$, which is called the {\em output-polynomial time}.
Hence, they are expected to run in practical time 
as long as $|\mathcal{P}|$ is small.
%even when $d$ is large, and $|\mathcal{P}|$ is exponentially large in the worst case.

\subsection*{Extension to Weighted FIM}
Standard FIM methods handle transactions as if there were no difference in 
importance among transactions. 
However, there often appear such cases
that importance may differ one another depending on transactions.
Actually, the values of importance may be positive and negative.
If each transaction is allocated to a positive or negative label,
then we may be interested in discovering itemsets that frequently appear in positive transactions and
not frequently in negative ones.

In the setting where only the positive importance is available,
we can utilize the backtracking algorithm or the apriori algorithm.  
An efficient 
algorithm can be constructed, since the monotonicity of frequent itemsets still holds.
We define {\it weighted frequency} as follows:
\begin{align}
\mathrm{frq}(p;\mathcal{T},\alpha) \triangleq \sum_{ t \in \mathcal{T}(p)} \alpha_t.
\end{align}
for given $\alpha_t$ for $t\in \mathcal{T}$.
The same monotonicity as \eqref{eq:monotonicity} still holds for the weighted variant of frequencies.
We are then led to non-negatively-weighted FIM. 
It is to find all itemsets with larger weighted frequency than a given threshold.

In the setting where both positive and negative importance has to be dealt with,
the monotonicity  does not hold any longer.
Then any algorithm of output-polynomial time may not exist.
However, we may instead employ the following two-stage strategy:
%It is known to be executable for practical use;
Let the sets of positive and negative transactions in $\mathcal{T} $ be $\mathcal{T}_+ $ and $\mathcal{T}_- $, respectively.
In the first stage, ignoring transactions with negative importance, we obtain frequent itemsets such that 
\begin{align}
\mathcal{P}_+ = \{p\subseteq \mathcal{I}\ |\ \mathrm{frq}(p ; \mathcal{T}_+, \alpha )>\theta\}.
\end{align}
In the second stage,  for each itemset in $\mathcal{P}_+$ we check if the frequency $\mathrm{frq}(p ; \mathcal{T})$ 
is still larger than $\theta$. 

The first stage is executed using 
the aforementioned algorithms in time  $\mathcal{O}(m\|\mathcal{T}_+\||\mathcal{P_+}|)$ 
while the second stage is executed in time
 $\mathcal{O}(m\|\mathcal{T_-}\||\mathcal{P_+}|)$ by accessing all negative transactions for each itemset obtained in 
the first stage. 
Then the total computation time is $\mathcal{O}(m\|\mathcal{T}\||\mathcal{P}_+|)$. 
The three types of FIM: standard FIM, non-negatively weighted FIM,  and weighted FIM are illustrated in Figure~\ref{fig:fim}.

\textcolor{red}{
%Note that we easily extend FIM (WFIM)
%kの上限…
WFIMのアルゴリズムをマイナーチェンジすることで、アイテム集合サイズに上限~$k$を与えた下でWFIMを実行可能である。
すなわち、$\mathcal{P}=\{p\subseteq \mathcal{I}\ |\ \mathrm{frq}(p;\mathcal{T},\alpha), |p|\leq k\}$
を出力することができる。
これは頻出アイテム集合を幅優先、深さ優先で探索する際、深さ~$k$に達したら探索を打ち切ることで実現されることから明らかである。
}

\if 0
頻出アイテム集合マイニングはデータマイニングの分野においての最も基本的な問題の一つであり，
アソシエーションルールマイニングなど多くの応用がある．

\paragraph{アプリオリ法}
アプリオリ法はAgrawal and Srikant~\cite{Agrawal94}によって初めて提案された．
アルゴリズム~\ref{algo:apriori}にアプリオリ法を示す．
\begin{algorithm}[!h]
\caption{アプリオリ法}
\label{algo:apriori}
\begin{algorithmic}[1]
\REQUIRE $\theta$：閾値
\STATE $\mathcal{P}_1\leftarrow\text{サイズ1の頻出集合の族}$
\STATE $k\leftarrow 1$
\WHILE {$\mathcal{P}_k\not=\emptyset$}
\STATE $\mathcal{P}_{k+1}\leftarrow(\text{$\mathcal{P}_k$の2つのアイテム集合の和集合でサイズが$k+1$の集合からなる族})$
\STATE $\forall p\in \mathcal{P}_{k+1}, \mathrm{frq}(p)<\theta$を$\mathcal{P}_{k+1}$から取り除く．
\STATE $k\leftarrow k+1$
\ENDWHILE
\STATE \textbf{output} $\mathcal{P}_1,\ldots,\mathcal{P}_{k-1}$
\end{algorithmic}
\end{algorithm}

アプリオリ法の時間計算量について考える．
アプリオリ法のステップ~5における$\mathcal{P}_{k+1}$の各アイテム集合の頻出度の計算に関しては，
アルゴリズム~\ref{algo:calc_freqs}を適用することで，データベースのスキャン1回のみで実行可能である．

\begin{algorithm}[!h]
\caption{頻出度の計算}
\label{algo:calc_freqs}
\begin{algorithmic}[1]
\REQUIRE $\mathcal{T}$：トランザクションデータベース，$\mathcal{P}_{k+1}$：アプリオリ法におけるサイズ~$k+1$の頻出アイテム集合の候補の族
\FORALL {$p\in\mathcal{P}_{k+1}$}
\STATE $\mathrm{frq}(p)\leftarrow 0$
\ENDFOR
\FORALL {$t\in\mathcal{T}$}
\FORALL {$p\in\mathcal{P}_{k+1}$}
\IF {$p\subseteq t$}
\STATE $\mathrm{frq}(p)\leftarrow \mathrm{frq}(p) + 1$
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\paragraph{バックトラック法}
バックトラック法のアルゴリズムを示す前に用語を導入する．
アイテム集合~$X$に対して，$X$中の最大のアイテムを\emph{末尾}（tail）と呼び$\mathrm{tail}(X)$と表す．
ただし$\mathrm{tail}(\emptyset)=-\infty$と定義する．
例えば$\mathrm{tail}(\{1,2,7\})=7$である．
また，アイテム集合~$X$をアイテム集合~$X-\{\mathrm{tail}(X)\}$から生成することを\emph{末尾拡張}（tail extension）と呼ぶ．
例えばアイテム集合~$\{1,2,4,7\}$は$\{1,2,4\}$の末尾拡張である．

末尾拡張を用いてバックトラック法が得られる．
アルゴリズム~\ref{algo:backtracking}にバックトラック法を示す．
バックトラック法は再帰的に定義されており，$\mathrm{Backtracking}(\emptyset)$を計算することで
全ての頻出アイテム集合が出力される．
\begin{algorithm}[!h]
\caption{$\mathrm{Backtracking}(X)$}
\label{algo:backtracking}
\begin{algorithmic}[1]
\REQUIRE $\theta$：閾値
\STATE \textbf{output} $X$
\FORALL {$i>\mathrm{tail}(X)$}
\IF {$\mathrm{frq}(X\cup\{i\})\geq\theta$}
\STATE $\mathrm{Backtracking}(X\cup\{i\})$
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}

バックトラック法の時間計算量について考える．
バックトラック法において頻出度~$\mathrm{frq}(\cdot)$の計算は各頻出アイテム集合の末尾拡張の合計回だけ行われる．
またある頻出アイテム集合~$X$に対してその末尾拡張は高々~$n$個であり，1回の頻出度の計算には~$\mathcal{O}(\|\mathcal{T}\|)$
かかるので，合計で$\mathcal{O}(n\|\mathcal{T}\||\mathcal{P}|)$時間でありアプリオリ法と同様となる．
\fi



==> grafting_0215.tex <==

\section{Grafting Algorithm}
\label{sec:grafting}

In this section we introduce grafting algorithm proposed by ~\citep{Perkins03}.
The grafting algorithm is proposed for solving large-scale regularized loss minimization problem
by constructing a set of active features by adding features incrementally.
In each iteration of grafting algorithm, a gradient-based heuristics find the feature that seemingly improve
the model most effectively to add it to the set of active features.

 In case we assume 
that there are redundant coordinates in the parameter vector $\bm{w}$ and $p$ is large,
we often use namely L1 regularizer for the part of $\Omega$.  The grafting algorithm 
is able to efficiently obtain a solution in such cases, i.e., in case $G$ is written as 
\begin{align}
\label{eq:L1}
 G(\bm{w}) = C \sum_{i=1}^m{ \ell \rbr{f_{\bm{w}}(\bm{x}_i ) , y_i}} + \nbr{\bm{w}}_1.
\end{align}
The basic strategy of grafting algorithm is to optimize the function incrementally 
as it is assumed to be more efficient when the optimal solution is sparse.
At each iteration of the grafting algorithm, a fast gradient-based heuristic is used to evaluate
which feature is seemingly most effective to decrease the objective function value according to the existing model.

At $t$-th iteration in the grafting algorithm, we can divide all components of parameter vector $\bm{w}$
into two distinct sets, $F^t$ and $Z^t\triangleq \neg F^t$. We call $w_j \in F^t$ free weights and we 
assume $w_j =0$ if $w_j \in Z^t$. We further assume \ref{eq:L1} is minimized with respect to free weights, i.e., we assume
\begin{align}
 　\partial_{w_j}G \ni 0 
\end{align}
for $\forall j\in F^t$. Here $ 　\partial_{w_j}G $ is subdifferential of $G$ with respect to $w_j$. 
On the other hand, for $\forall j\in Z^t$, 
\begin{align}
  \label{eq:cond}
 　\partial_{w_j}G \not\ni 0 
\end{align}
is a necessary and sufficient condition to decrease the objective function value by
changing the value of $w_j$ globally in case of convex $G$ and locally in general. 
For the parameter $w_j\in Z^t$, the subdifferential can be computed as following:
\begin{align}
\nonumber
\partial_{w_j}G 
&= 
\bigg\{c\ \bigg|
C\sum_{i=1}^m
\left(\frac{\partial \ell}{\partial f_{\bm{w}}(\bm{x}_i)}\frac{\partial f_{\bm{w}}(\bm{x}_i)}{\partial w_j}\right) - 1 \le c, \\
&
\nonumber 
\phantom{.....\bigg\{c\ \bigg| }
C\sum_{i=1}^m
\left(\frac{\partial \ell}{\partial f_{\bm{w}}(\bm{x}_i)}\frac{\partial f_{\bm{w}}(\bm{x}_i)}{\partial w_j}\right) + 1 \ge c \ \, \bigg\} \\
\label{eq:subdiff}
&= \left\{c\ \middle| \frac{\partial L}{\partial w_j} - 1 \le c \le \frac{\partial L}{\partial w_j} + 1 \right\} ,
\end{align}
where we defined $L(\bm{w})\triangleq\sum_{i=1}^m\ell(f_{\bm{w}}(\bm{x}_i),y_i)$.
Therefore the condition~\eqref{eq:cond} is reduced to 
\begin{align}
\label{eq:subdiff_cond}
\left|\frac{\partial L}{\partial w_j}\right| > 1.
\end{align}
This also indicates changing the value of $w_j$ from 0 
will not decrease the objective function value 
of the current mode,l given that \eqref{eq:subdiff_cond} is not satisfied.
This is the essential reason that $L_1$ regularization motivates sparese
solution and gives stopping condition of the grafting algorithm as we describe in
the section below.

\subsection*{Parameter selection}
We consider to select a parameter to move from $Z^t$ to $F^t$.
By the arguments above, we see that such $w_j\in Z^t$ that satisfies 
\eqref{eq:subdiff_cond} can make the objective function value decrease by 
changing the value from 0. However, multiple candidates that
satisfies \eqref{eq:subdiff_cond} can exist in some cases.
Expecting to make objective function decrease most largely, the 
grafting algorithm selects a parameter $w_{\mathrm{best}}$
by following gradient-based heuristics:
\begin{align}
\label{eq:grafting_weight_choice}
w_{\mathrm{best}}=\argmax_{w_j\in Z^t} \left|\frac{\partial L}{\partial w_j}\right|，
\end{align}
In general learning model, there is no efficient way for the computing this selecting rule
and basically requires to compute derivatives with respect to all parameters to obtain 
the maximum in \eqref{eq:subdiff_cond}.
Note that this computation therefore easily becomes impractical in case 
the number of instances and components of parameters is of large-scale in general.

\subsection*{Stopping condition}
In case that the condition \eqref{eq:subdiff_cond} is not satisfied
for all $w_j\in Z^t$, objective function value cannot be decreased
by changing the value of $w_j\in Z^t$ from 0 the value of 
$w_j\in F^t$ from current value, globally in case of convex $G$ and 
locally in general case.
Therefore this can be used as a stopping condition of the grafting
algorithm, as it indicates that local optimum and global optimum
in case of convex $G$ is achieved.


\subsection*{Entire procedure}
Overall procedure of the grafting algorithm becomes as follows:
first we compute $w_j$ that maximizes $|\partial L/\partial w_j|$ among all $w_j\in Z$,
secondly we add it to the set of free weights and optimize \eqref{eq:L1} with respect to $w_j\in F^t$.
Note that the optimization can be significantly efficient by performing warm-start by the optimal
solution at the previous iteration. Also we note that 
the selection according to $|\partial L/\partial w_j|$ will not necessarily select
the optimal parameter, although we can be more efficient than selecting one randomly.
The procedure is described in algorithm~\ref{algo:grafting}.

\begin{algorithm}[!tb]
\caption{The grafting algorithm for $L_1$ regularization problem}
\label{algo:grafting}
\begin{algorithmic}[1]
\REQUIRE $G(\bm{w})=L(\bm{w})+\lambda \|\bm{w}\|_1$
\STATE $F^0\leftarrow\emptyset, Z^0\leftarrow \{w_j\}_{j=1}^p,t\gets 0$
\WHILE {$\max_{w_j \in Z} \left|\partial L/\partial w_j\right|>\lambda$}
  \STATE $w_j\leftarrow \argmax_{w_j\in Z} \left|\partial L/\partial w_j\right|$
  \STATE $F^{t+1}\gets F^t \cup \{w_j\} $;\ $Z^{t+1}\gets Z^t \setminus \{w_j\} $
  \STATE $t \gets t+1$
  \STATE Optimize $G(\bm{w})$ with respect to $\forall w_j\in F$
\ENDWHILE
\end{algorithmic}
\end{algorithm}



==> grafting_0217.tex <==
\section{Grafting Algorithm}
\label{sec:grafting}

In this section we introduce the grafting algorithm~\citep{Perkins03},
which is designed for solving large-scale regularized loss minimization problem.
The key idea of the grafting algorithm is to construct a set of active features by adding features incrementally.
In each iteration of the grafting algorithm, a gradient-based heuristics  is employed to find the feature that seemingly improve
the model most effectively and to add it to the set of active features.

Suppose that the data dimension is so large enough that there are too many irrelevant attributes in the parameter vector $\bm{w}$. 
Then we may employ the L1 regularizer  as the penalty term $\Omega$ in 
(\ref{eq:ERM}). 
The grafting algorithm is designed so that it can solve the optimization problem efficiently for this case. 
Then $G$ is written as 
\begin{align}
\label{eq:L1}
 G(\bm{w}) = C \sum_{i=1}^m{ \ell \rbr{f_{\bm{w}}(\bm{x}_i ) , y_i}} + \nbr{\bm{w}}_1.
\end{align}
The grafting algorithm optimizes this objective function iteratively.
%as it is assumed to be more efficient when the optimal solution is sparse.
At each iteration, a gradient-based heuristic is employed to determine
which feature is most effective for decreasing  the objective function.
%  according to the existing model.

At the $t$-th iteration, the grafting algorithm divides all of the attributes of parameter vector $\bm{w}$
into two disjoint sets, $F^t$ and $Z^t\triangleq \neg F^t$. We call $w_j \in F^t${
{\em free weights}.  
Set $w_j =0$ if $w_j \in Z^t$. 
It minimizes (\ref{eq:L1})  with respect to free weights, assuming that
\begin{align}
\label{eq:cond_weights_in_f}
 　\partial_{w_j}G \ni 0 
\end{align}
for $\forall j\in F^t$, where $ 　\partial_{w_j}G $ is a partial differential of $G$ with respect to $w_j$. 
On the other hand, for $\forall j\in Z^t$, 
\begin{align}
  \label{eq:cond}
 　\partial_{w_j}G \not\ni 0 
\end{align}
is a necessary and sufficient condition for the value of the objective function to decrease by 
changing the  $w_j$.
%It decreases globally in case of convex $G$ and locally in general. 
The partial differential of the objective function with respect to  $w_j\in Z^t$
is calculated as follows:
\begin{align}
\nonumber
\partial_{w_j}G 
&= 
\bigg\{c\ \bigg|
C\sum_{i=1}^m
\left(\frac{\partial \ell}{\partial f_{\bm{w}}(\bm{x}_i)}\frac{\partial f_{\bm{w}}(\bm{x}_i)}{\partial w_j}\right) - 1 \le c, \\
&
\nonumber 
\phantom{.....\bigg\{c\ \bigg| }
C\sum_{i=1}^m
\left(\frac{\partial \ell}{\partial f_{\bm{w}}(\bm{x}_i)}\frac{\partial f_{\bm{w}}(\bm{x}_i)}{\partial w_j}\right) + 1 \ge c \ \, \bigg\} \\
\label{eq:subdiff}
&= \left\{c\ \middle| \frac{\partial L}{\partial w_j} - 1 \le c \le \frac{\partial L}{\partial w_j} + 1 \right\} ,
\end{align}
where $L(\bm{w})\triangleq\sum_{i=1}^m\ell(f_{\bm{w}}(\bm{x}_i),y_i)$.
Hence the condition~\eqref{eq:cond} is equivalent with 
\begin{align}
\label{eq:subdiff_cond}
\left|\frac{\partial L}{\partial w_j}\right| > 1.
\end{align}
This implies that changing the value of $w_j$ from $0 $
will not decrease the value of the objective function  if \eqref{eq:subdiff_cond} is not satisfied.
This is the main reason why $L_1$ regularization gives  a sparse
solution. It also leads to a stopping condition of the grafting algorithm as shown below.

\subsection*{Parameter selection}
We consider the problem of  selecting a parameter to move from $Z^t$ to $F^t$.
We see from the above argument that $w_j\in Z^t$ satisfying
\eqref{eq:subdiff_cond} makes the  value of the objective function  decrease by 
changing its value from $0$. 
There may exist more than one candidates that
satisfies \eqref{eq:subdiff_cond}.
In that case, the grafting algorithm selects a parameter~$w_{\mathrm{best}}$ that makes the 
value of the objective function decrease most, by making use of the following 
gradient-based heuristics:
\begin{align}
\label{eq:grafting_weight_choice}
w_{\mathrm{best}}=\argmax_{w_j\in Z^t} \left|\frac{\partial L}{\partial w_j}\right|,
\end{align}
For general models, 
the derivatives of the objective function with respect to all parameters must be calculated to obtain 
the maximum in \eqref{eq:subdiff_cond}.
However, this na\"{i}ve method might be  computationally intractable when 
the data dimension and sample size are of large-scale.
To the best of  the authors' knowledge, there does not exit any  efficient method for conducting this parameter selecting rule. 

\subsection*{Stopping condition}
If the condition \eqref{eq:subdiff_cond} is not satisfied
for all $w_j\in Z^t$, the value of the objective function is not decreased
by changing the value of $w_j\in Z^t$ from $0$ and the value of 
$w_j\in F^t$ from the current value, globally in case of convex $G$ and 
locally in general cases.
Therefore this condition can be used as a stopping condition for the grafting
algorithm, as it indicates that local optimum (or the global optimum
in case of convex $G$) is achieved.


\subsection*{Entire procedure}
We describe the overall procedure of the grafting algorithm as follows:
First we compute $w_j$ that maximizes $|\partial L/\partial w_j|$ among all $w_j\in Z$.
Secondly we add it to the set of free weights and optimize \eqref{eq:L1} with respect to $w_j\in F^t$.
Note that the optimization can be conducted efficiently by warm-starting from the optimal
solution at the previous iteration. 
Note here that 
the parameter selection procedure using the value of $|\partial L/\partial w_j|$ will not necessarily select
the optimal parameter.
%, although we can be more efficient than selecting one randomly.
The procedure is given in Algorithm~\ref{algo:grafting}.

\begin{algorithm}[!tb]
\caption{The grafting algorithm for $L_1$ regularization problem}
\label{algo:grafting}
\begin{algorithmic}[1]
\REQUIRE $G(\bm{w})=L(\bm{w})+\lambda \|\bm{w}\|_1$
\STATE $F^0\leftarrow\emptyset, Z^0\leftarrow \{w_j\}_{j=1}^p,t\gets 0$
\WHILE {$\max_{w_j \in Z} \left|\partial L/\partial w_j\right|>\lambda$}
  \STATE $w_j\leftarrow \argmax_{w_j\in Z} \left|\partial L/\partial w_j\right|$
  \STATE $F^{t+1}\gets F^t \cup \{w_j\} $;\ $Z^{t+1}\gets Z^t \setminus \{w_j\} $
  \STATE $t \gets t+1$
  \STATE Optimize $G(\bm{w})$ with respect to $\forall w_j\in F$
\ENDWHILE
\end{algorithmic}
\end{algorithm}



==> proposed_0217.tex <==
\section{Proposed Algorithm (GRAB) }
\label{sec:grab}

In this section we introduce our proposed algorithm for learning CBM, 
which we call GRAB (GRAfting for Boolean datasets).
As shown in Section~\ref{sec:combinatorial_boolean_model}, CBM has at most $2^d$ parameters. 
It is difficult to store all the values $\phi(\bm{x}_i)$ for all $\phi$ and $i$ from the viewpoint of space complexity. Further, it is difficult to 
solve this large-scale optimization problem from the viewpoint of time complexity.
However, we can overcome these difficulties by using the grafting algorithm in combination with the weighted FIM, which we abbreviate as WFIM.
Let us consider to solve the optimization problem for learning CBM by means of the grafting algorithm.
It can overcome the space complexity issue because it does not require that all the possible features be stored.
On the other hand, a time complexity issue arises
in the process of finding a new feature in each iteration.

The subdifferential of the objective function~$G^{(k)}$ with respect to $w_\phi$ is given as follows:
\begin{align*}
\partial_{w_\phi}G 
&= 
\bigg\{c\ \bigg|
C\sum_{i=1}^m
\left(\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)}\frac{\partial f^{(k)}(\bm{x}_i)}{\partial w_\phi}\right) - 1 \le c, \\
&
\phantom{.....\bigg\{c\ \bigg|}
C\sum_{i=1}^m
\left(\frac{\partial \ell}{\partial f_{\bm{w}}(\bm{x}_i)}\frac{\partial f_{\bm{w}}(\bm{x}_i)}{\partial w_\phi}\right) + 1 \ge c \ \, \bigg\} \\
&=
\bigg\{c\ \bigg|
C\sum_{i=1}^m
\left(\frac{\partial\ell}{\partial f^{(k)}(\bm{x}_i)}\phi(\bm{x}_i)\right) - 1 \le c, \\
&
\phantom{.....\bigg\{c\ \bigg|}
C\sum_{i=1}^m
\left(\frac{\partial\ell}{\partial f^{(k)}(\bm{x}_i)}\phi(\bm{x}_i)\right) + 1 \ge c \ \, \bigg\}.
\end{align*}
We see from \eqref{eq:subdiff_cond} that the value of the objective function is  decreased by 
changing the value of $w_\phi$ if and only if
\begin{align}
\label{eq:grab_cond11}
\left|C\sum_{i=1}^m\left(\frac{\partial L}{\partial f^{(k)}(\bm{x}_i)}
\phi(\bm{x}_i)\right)\right| > 1.
\end{align}
Thus, the problem of finding the best feature in the sense of grafting algorithm as in \eqref{ } is reduced
to finding $\phi \in \Phi^{(k)}$ that maximizes the left hand side of \eqref{eq:grab_cond11}.

To solve this problem, we utilize the technique of WFIM for finding parameters satisfying \eqref{eq:grab_cond11}.
Note that the feature vector~$\bm{x}$ is an element of $\{0,1\}^d$.
Let us define a bijection~$T^{(d)}(\cdot)$ from ~$\{0,1\}^d$ to $2^{\{1,2,\ldots,d\}}$
and an injection~$P^{(k)}(\cdot)$ from $\Phi^{(k)}$ to $2^{\{1,2,\ldots,d\}}$
as follows:
\begin{align*}
T^{(d)}(\bm{x}) &= \{k\mid x_k=1\ (k=1,\ldots, d)\}, \\
P^{(k)}(\phi)&=\left\{ \begin{array}{lr}
\emptyset & (\phi = \top(\bm{x})), \\
\{i_1,\ldots,i_l\} & (\phi = x_{i_1}\wedge\ldots\wedge x_{i_l}).
\end{array}
\right.
\end{align*}
Using these functions, it holds that
\begin{align*}
\phi(\bm{x}) &= \left\{\begin{array}{lr}
1 & (T^{(d)}(\bm{x})\supset P^{(k)}(\phi)) ,\\
0 & (\text{otherwise.}).
\end{array}\right.
\end{align*}
We abbreviate $T^{(d)}(\bm{x}_i)$ and $P^{(k)}(\phi)$ as $t_i$ and $p_\phi$, respectively,
for each feature vector~$\bm{x}_i\ (i=1,\ldots,m)$ and $\phi\in\Phi^{(k)}$.
The left-hand side of \eqref{eq:grab_cond11} is rewritten as
\begin{align*}
\left|C\sum_{i=1}^m\left(\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)}
\phi(\bm{x}_i)\right)\right| &= 
\left|C\sum_{\{i\ |\ \phi(\bm{x}_i)=1\}}\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)}\right| \\
&=\left|C\sum_{\{i\ |\ t_i \supseteq\ p_\phi \}}\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)}\right| \\
&=\left|C\sum_{\{i\ |\ t_i\in \mathcal{T}(p_\phi ) \}}\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)}\right|,
\end{align*}
where $\mathcal{T}(p_\phi )$ is an occurence set of $p_\phi$ with respect to the transaction database 
$\mathcal{T}$ that regards $t_i$ as each transaction for $i=1,\ldots,m$.
Hence, we see \eqref{eq:grab_cond11} is rewritten as
\begin{align}
\mathrm{frq}(p_\phi ; \mathcal{T}, \alpha) > 1 
\label{eq:grab_cond_pos_neg} 
\quad \text{or} \quad
%\label{eq:grab_cond_neg}
\mathrm{frq}(p_\phi ; \mathcal{T} , -\alpha) > 1,
%\sum_{\{i\ |\ z_i\supset p_\phi\}}-C\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)} &> 1.
\end{align}
where
\begin{align}
\label{eq:transaction_weights}
\alpha_{t_i} = C\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)} .
\end{align}
%In the context of FIM,
%$\sum_{\{i\ |\ z_i\supset p_\phi\}}$ can be interpreted as the procedure
%that takes sum for $i$ such that the transaction~$z_i$ has the occurrence of the itemset~$p_\phi$.
In other words,
we can obtain all $p_\phi$ that satisfy \eqref{eq:grab_cond_pos_neg}
by employing WFIM for the transaction database~$\mathcal{T}$
and the transaction weights as in~\eqref{eq:transaction_weights}
to obtain a set of all $p_\phi$s satisfying \eqref{eq:grab_cond_pos_neg}.
According to the original form of grafting algorithm, only one parameter is newly added to free weights
by \eqref{eq:grafting_weight_choice} at each iteration.
However, knowing that \eqref{eq:grab_cond11} is a sufficient and necessary condition for the 
objective function to decrease, we may select more than one  parameters such as selecting 
the top-K frequent parameters: $\{w_{\phi _{i}}\}_{i=1}^{K}$ where $p_{\phi _{i}}$ is the $i$-th most frequent itemset in $\mathcal{P}$. 
This method is more efficient when the parameter selection procedure of WFIM requires much computation time
than parameter estimation step of the grafting algorithm.

The overall flow of GRAB algorithm is given in Algorithm~\ref{algo:grab}.
\textcolor{red}{
Let us discuss the time complexity of GRAB algorithm.
At each step of GRAB, we perform WFIM and optimization of $G^{(k)}(\bm{w})$.
Since time complexity for the optimization largely depends on the loss function of CBM and the employed solver,
we only consider time complexity for WFIM step.
It can be considered, however, that WFIM takes much more time than the optimization in many cases.
As discussed at Section~\ref{sec:fim}, the computation time of WFIM is $\mathcal{O}\rbr{n\nbr{\mathcal{T}}|\mathcal{P}_+|}$.
Here, it obviously holds that $\mathcal{P}_+\subseteq \mathcal{P}_\mathrm{all}$,
where $\mathcal{P}_\mathrm{all}\triangleq\{p\subseteq\mathcal{I}\ |\ \mathrm{frq}\rbr{p;\mathcal{T}}>0\}$.
Since we move at least one parameter from $Z^t$ to $F^t$ at $t$-th GRAB step,
it also holds that $T<|\mathcal{P}_\mathrm{all}|$, where $T$ is the total number of iterations of GRAB.
Using these relationships, the total computation time for WFIM step in GRAB can be evaluated as follows:
\begin{align*}
\sum_{t=1}^T \mathcal{O}\rbr{n\nbr{\mathcal{T}}|\mathcal{P}_+^{(t)}|}&=
T\times\mathcal{O}\rbr{n\nbr{\mathcal{T}}|\mathcal{P}_\mathrm{all}|} \\
&= \mathcal{O}\rbr{n\nbr{\mathcal{T}}|\mathcal{P}_\mathrm{all}|^2}.
\end{align*}
}

\begin{algorithm}[!tb]
\caption{GRAB algorithm}
\label{algo:grab}
\begin{algorithmic}[1]
\INPUT $k\ge 0, \{\bm{x}_i ,y_i\}_{i=1,\ldots,m}, C>0$
\REQUIRE $
%G^{(k)}(\bm{w})=C\sum_{i=1}^m L\left(\sum_{\phi\in\Phi^{(k)}}w_\phi \phi(\bm{x}_i),y_i\right)+\|\bm{w}\|_1, \ \ \  
\mathcal{T} = \cbr{t_i}_{i=1,\ldots,m}
$
\STATE $t_i \gets T^{(d)} (\bm{x}_i), \ \alpha_{t_i} \gets C\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)}  \quad ( i =1,\ldots,m) $
\STATE $\mathcal{P} \gets \cbr{\ p\  | \  \mathrm{frq}(p_\phi ; \mathcal{T}, \alpha) > 1 \ \text{or} \ \mathrm{frq}(p_\phi ; \mathcal{T} , -\alpha) > 1, |p| \le k}$
\STATE $F\leftarrow\varnothing, Z\leftarrow \{w_\phi\}_{\phi\in\Phi^{(k)}}$
\WHILE {$\mathcal{P}\not=\varnothing$}
%  \STATE $\phi\leftarrow\left(P^{(k)}\right)^{-1}(p_{\max})\ (p_{\max}\text{is the most frequent itemset in $P$.})$
  \FOR{$j=1,\ldots,K$ }
  \STATE Pick $\phi$ such that $p_{\phi}$ is the $j$-th most frequent itemset in $\mathcal{P}$
  \STATE Move $w_{\phi}$ to $F$ from $Z$.
  \ENDFOR
  \STATE Optimize $G^{(k)}(\bm{w})$ w.r.t. $w_\phi\in F$
  \STATE $\alpha_{t_i} \gets C\frac{\partial \ell}{\partial f^{(k)}(\bm{x}_i)} $
  \STATE $\mathcal{P} \gets \cbr{\ p\  | \  \mathrm{frq}(p_\phi ; \mathcal{T}, \alpha) > 1 \ \text{or} \ \mathrm{frq}(p_\phi ; \mathcal{T} , -\alpha) > 1, |p| \le k}$
\ENDWHILE
\OUTPUT $\{w_\phi\}_{\phi\in F}$
\end{algorithmic}
\end{algorithm}

\subsection*{Implementation Issue}
\textcolor{red}{
We describe implementation details concerned with acceleration 
and termination of the proposed algorithm.
\paragraph{Dynamic threshold control for the acceleration of WFIM}
As we have seen that the time complexity of WFIM is described as 
$\Ocal(n\|\mathcal{T}\||\mathcal{P}_+|)$,
WFIM terminates faster as threshold $\theta$ is set to a larger value and $|\mathcal{P}_+|$ gets smaller.
In order to obtain top-$K$ frequent itemsets without extracting all the feature that satisfies \eqref{eq:grab_cond11}, 
we first executed WFIM by setting the threshold $\theta = 2^M$ with $M=10$,
and decrement $M$ by $1$ until we obtain $K$ itemsets or it becomes $\theta=2^0=1$.
When WFIM is called next time, we used the same value of $M$ as that previously used.
}

\textcolor{red}{
\paragraph{Incomplete Termination of WFIM}
When the output of WFIM is too large even after setting threshold dynamically,
we terminated WFIM after extracting $100K$ frequent itemsets and
selected top-$K$ frequent itemsets among those.
In such cases, we no longer have guarantee for selecting top-$K$ frequent itemsets.
However, as the condition on drawing a new feature based on \eqref{eq:grafting_weight_choice}
is already a heuristic choice, we consider it does not deteriorate the performance
of proceeding optimization step significantly.
}

\textcolor{red}{
\paragraph{Stopping condition}
We employ a stopping condition as follows. First we define the suboptimality of 
the solution as follows:
\begin{align*}
V^{(t)}&=\sum_{\phi\in\Phi^{(k)}}\max\left(C\left|\frac{\partial L}{\partial w_\phi^{(t)}}\right| - 1, 0\right) \\
	   &=\sum_{\phi\in F^t}\max\left(C\left|\frac{\partial L}{\partial w_\phi^{(t)}}\right| - 1, 0\right)
       +\sum_{\phi\in Z^t}\max\left(C\left|\frac{\partial L}{\partial w_\phi^{(t)}}\right| - 1, 0\right).
\end{align*}
Then,  given a tolarence $\varepsilon>0$, 
we terminate the algorithm when $V^{(t)} < \varepsilon V^{(0)}$ is satisfied.
The first term of $V^{(t)}$ can be computed by the parameter obtained by the optimization step
and the second is computed by summing over features obtained by WFIM.
$V^{0}$ often cannot be computed exactly as the we employ the acceleration techniques
described above. We underestimated $V^{(0)}$ by computing the summand in the second term
among obtained features. This makes stopping condition stricter and the proposed algorithm run longer.
In our experiments, we set $\varepsilon=0.01$.
}

\if 0
\textcolor{red}{
アルゴリズム~\ref{algo:grab}からわかる通り、GRABの停止条件はWFIMの出力が空集合になった時であるが、
計算機上では第7ステップにおいて$G^{(k)}(\bm{w})$を最適化した後、式~\eqref{eq:cond_weights_in_f}が
厳密には満たされないという問題がある。
そこで、LIBLINEARなどで用いられているアルゴリズムに習い、次のような停止条件を与える。
まず第~$t$ステップにおけるパラメータを$\bm{w}^{(t)}=\{w_\phi^{(t)}\}_{\phi\in\Phi^{(k)}}$とし、微分値の残差~$V^{(t)}$を次式で与える。
\begin{align*}
V^{(t)}&=\sum_{\phi\in\Phi^{(k)}}\max\left(C\left|\frac{\partial L}{\partial w_\phi^{(t)}}\right| - 1, 0\right) \\
	   &=\sum_{\phi\in F^t}\max\left(C\left|\frac{\partial L}{\partial w_\phi^{(t)}}\right| - 1, 0\right)
       +\sum_{\phi\in Z^t}\max\left(C\left|\frac{\partial L}{\partial w_\phi^{(t)}}\right| - 1, 0\right)
\end{align*}
これを用いてアルゴリズムの終了条件を$0<\epsilon<1$を与えた下で、$V^{(t)}/V^{(0)} <\epsilon$を満たした時と定める。
$V^{(t)}$の第一項に関しては、アルゴリズム~\ref{algo:grab}の第7ステップ後のパラメータから計算でき、
第二項に関しては式~\eqref{eq:grab_cond11}より、WFIMによって出力された$\phi\in\Phi^{(k)}$についてのみ和を取れば良い。
実際にはThreshold controlとBatch extractionを利用しているため、$V^{(0)}$の正確な計算はできず$V^{(0)}$より小さい値を
得ることになるが、その場合でも終了条件が厳しいものになるだけなので問題にはならない。
}
\fi
\subsection*{Related Work}
Frequent Itemset Mining is used for machine learning in 
several other tasks such as clustering and boosting \citep{Saigo07,Tsuda06,Kudo04}.
\\
Our application is non-tribial

